FlowSense: Monitoring Airflow in Building Ventilation Systems Using Audio Sensing

Proper indoor ventilation through buildings' heating, ventilation, and air conditioning (HVAC) systems has become an increasing public health concern that significantly impacts individuals' health and safety at home, work, and school. While much work has progressed in providing energy-efficient and user comfort for HVAC systems through IoT devices and mobile-sensing approaches, ventilation is an aspect that has received lesser attention despite its importance. With a motivation to monitor airflow from building ventilation systems through commodity sensing devices, we present FlowSense, a machine learning-based algorithm to predict airflow rate from sensed audio data in indoor spaces. Our ML technique can predict the state of an air vent-whether it is on or off-as well as the rate of air flowing through active vents. By exploiting a low-pass filter to obtain low-frequency audio signals, we put together a privacy-preserving pipeline that leverages a silence detection algorithm to only sense for sounds of air from HVAC air vent when no human speech is detected. We also propose the Minimum Persistent Sensing (MPS) as a post-processing algorithm to reduce interference from ambient noise, including ongoing human conversation, office machines, and traffic noises. Together, these techniques ensure user privacy and improve the robustness of FlowSense. We validate our approach yielding over 90% accuracy in predicting vent status and 0.96 MSE in predicting airflow rate when the device is placed within 2.25 meters away from an air vent. Additionally, we demonstrate how our approach as a mobile audio-sensing platform is robust to smartphone models, distance, and orientation. Finally, we evaluate FlowSense privacy-preserving pipeline through a user study and a Google Speech Recognition service, confirming that the audio signals we used as input data are inaudible and inconstructible.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> background.tex <==
\section{Motivation and Background}
\label{sec:background}
This section explains our motivation to leverage a microphone sensor to measure airflow in indoor spaces.
\newline
\newline
With humans spending much of our time indoors, healthy indoor air quality is a fundamental aspect of our health \cite{epa}. Ventilation basically requires pulling fresh air from outdoors into an indoor space and pushing stale air from the indoor space to outside of the building. Doing so helps regulate and displace the existing air pollutants, aiding indoor spaces to keep the air quality healthy. We carry out ventilation through natural means such as opening windows and using room-level fans to circulate air, to more advanced methods of installing air filtration systems such as portable HEPA filtration and Ultraviolet germicidal irradiation (UVGI) purification systems. 

Since the recent coronavirus outbreak, the World Health Organization (WHO), American Society of Heating, Refrigerating and Air-Conditioning Engineers (ASHRAE), and Centers for Disease Control and Prevention (CDC) have recommended more strict guidelines on outdoor air supply for indoor office environments in the United States \cite{ashraeOpen,cdc2019,world2021roadmap}. For example, when indoor spaces become heavily occupied and remain unventilated, these areas increase risk that breathe in the carbon dioxide, exhaled water vapor, and other impurities as exhaled air accumulates. 

\subsubsection*{Ventilation Guideline}
With airflow rate defined as the volume of air being ``delivered'' from one space to another, typically at a rate of cubic feet per minute (cfm), an occupant should receive approximately five cfm of outdoor air when indoor \cite{cdc2015}. One way to evaluate the sufficiency of airflow is through measuring CO\textsubscript{2} concentration, whereby CO\textsubscript{2} concentrations no more than 700 parts per million (ppm) above outdoor CO\textsubscript{2} concentrations are satisfactory for 80\% of indoor occupants \cite{cdc2015}. Another way is by measuring the rate of airflow through the air supply vents.

\subsubsection*{State-of-the-Art Airflow Sensors}
Advanced air-conditioning systems are typically installed with airflow sensing devices close to the cooling or heating system. These devices include air meters, pressure sensors, and vane anemometers \cite{sundell2011ventilation,taylor2003measurement, mcwilliams2002review}. While highly accurate, these modalities are typically hardwired devices and require commissioning providers to install and calibrate the sensors. This setup is more appropriate for facility managers to maintain an HVAC control system, but is not informative to everyday users about the airflow around them.
\newline
\newline
The motivation of our work sets in from the perspective of empowering users with critical healthy air information to make better decisions of what buildings to enter while assisting the organization stakeholder to maintain standards. Thus, airflow measurement needs to be enabled and accessible without dedicated devices and expert installation.


\subsection{Design Intuition}
Let us assume a standard HVAC operations schedule deployed in an office building. It makes its first run of air ventilation early in the morning when the building space is most likely unoccupied. The first ventilation schedule should introduce as much outside air as possible to reduce pollutants accumulated overnight. As the building becomes occupied,, indoor pollutants will increase the need to ventilate again. When an HVAC operation runs, occupants can typically hear ``noise'' coming from the air vent. However, the prominence of us hearing these noises varies with the ambient noise level in the room -- made up of human chatters, appliances, or even outdoor traffic. Indeed, these faint sounds of moving air from the air vents drive our curiosity in using them as a sensing modality; therefore, we seek an understanding in how this noise can be exploited to measure airflow as a data source. 

\subsection{Leveraging  Mobile Sensing}
Mobile sensing has been well established in the literature to provide vital information for air monitoring \cite{aram2012environment}. Some of these efforts include estimating ambient temperature through smartphone batteries \cite{breda2019hot}, determining human occupancy \cite{jiefan2018extracting} as a spatial characteristic to control HVAC ventilation, and estimating zone-based collaboration to calculate air exchange rate from temporal CO\textsubscript{2} concentration \cite{jiang2011maqs}. In the same vein, W-Air employs a low-cost gas sensor and wearable sensors to monitor indoor CO\textsubscript{2} concentrations \cite{maag2018w}. From reviewing prior work, one essential aspect of indoor air quality that we believe can benefit everyday users is recognizing how much air ventilation is required in the indoor space they are in. While this is not the central focus, determining airflow rate is the first step to realizing adequate indoor ventilation. We discuss this as part of our study implications in Section \ref{sec:discussion}.

\subsubsection{Air in Audio Sensing}
Conceptually, there is prior work related to air sensing. Many of these efforts are geared towards utilizing the microphone sensor but for sensing human respiration~\cite{kulkas2009intelligent,shih2019breeze, larson2012spirosmart}. For example, Wang et al. developed a respiration monitoring system by sensing audio signal changes during respiration \cite{wang2018c}. Nam et al. detected nasal breath sound recordings from a microphone built-in smartphones to estimate respiration rate \cite{nam2015estimation}. Fundamentally, these works employ different audio-processing methods to extract frequency content from (breathing) audio signals. First, they identify respiratory cycle phases in the signals and then eliminate irrelevant motion noises to estimate physiological measures \cite{larson2012spirosmart,song2020spirosonic}. 

These findings strengthen our decision of leveraging the same microphone sensor as a modality for collecting audio signals in the environment and estimating airflow within the space.

\subsection{Privacy in Audio Sensing}
Despite the increasing recognition capability in audio sensing, working with audio as a primary data source often raises privacy concerns. In the context of an audio processing system for measuring airflow, the system should not learn anything about the user's speech. 

Many researchers have proposed techniques that use inaudible signals to fulfill a system's functionality. For example, Sumeet et al. suggested randomly mutating raw sound frames and sub-sampling them to circumvent speech recovery \cite{kumar2015sound}. Other works include building speech classifiers and filtering these segments out when analyzing the core functionality, such as detecting coughs and breathing patterns \cite{ahmed2019mlung,liaqat2017method,larson2011accurate}. In the most recent study, Iravantchi et al. demonstrated how PrivacyMic takes advantage of inaudible frequencies to aid in acoustic activity recognition tasks \cite{iravantchi2021privacymic}. 

Overall the literature on utilizing inaudible frequencies indicates a promise to preserve user privacy when collecting audio signals. Thus, it led us to query if inaudible frequencies may also help measure airflow in the environment. Such knowledge could help pave the way for more accessible forms of airflow sensors.

\subsection{Summary}
The need for a low-cost and convenient airflow sensor to measure daily ventilation in indoor spaces motivates our work. Unlike prior research, which has established sensing mechanisms for airflow patterns in the respiratory tract, our work aims to sense moving air that can be quantified using ambient noise from ventilation systems. With this information, building occupants can be informed of the ventilation rate surrounding them. The choice of a microphone as a mode should take into account the practical considerations of user privacy and should be able to separate air from other ambient noise that exists within an overlapping frequency range.

==> backgroundMotivation.tex <==
\section{Motivation and Intuition}
\label{sec:background}
This section explains our motivation to leverage a microphone sensor and its feasibility to measure airflow in indoor spaces.
\newline
\newline
\noindent The motivation of our work sets in from the perspective of empowering users with critical healthy air information to make better decisions of what buildings to enter while assisting the organization stakeholder to maintain standards. With humans spending more than 90\% of their time indoors [X] and the recent COVID-19 outbreak exemplifying extreme health risks in poorly ventilated indoor spaces [X], measuring the airflow rate is fundamental in enabling proper ventilation to provide occupant comfort and safety [X].

\subsubsection*{General Practice and Guidelines}
Ventilation basically requires pulling fresh air from outdoors into an indoor space and pushing stale air from the indoor space to outside of the building. Doing so helps regulate and displace the existing air pollutants, aiding indoor spaces to keep the air quality healthy. We carry out ventilation through natural means such as opening windows and using room-level fans to circulate air to more advanced heating, ventilation, and air conditioning (HVAC) systems. Many HVAC systems in modern commercial buildings are typically installed with airflow sensing devices close to the ventilation duct. These devices include air meters, pressure sensors, and vane anemometers \cite{sundell2011ventilation,taylor2003measurement, mcwilliams2002review}. While highly accurate, these modalities are typically hardwired devices and require commissioning providers to install and calibrate the sensors. The setup is more appropriate for facility managers to maintain an HVAC control system, but is not informative to everyday users about the airflow around them.

\subsection{Design Intuition}
Since ushering in the era of informative health powered by mobile sensing, much research efforts have successfully created rich, open sensing environments where people and municipalities can acquire real-time access to environmental data. For example, estimating CO\textsubscript{2} footprint using GPS mobility data \cite{XXX} or predicting ambient air temperature through smartphone batteries \cite{aram2012environment,breda2019hot,devarakonda2013real, agarwal2011duty}. In the same vein, we believe mobile sensing holds the potential to measure the rate of airflow in real-time. However, measuring airflow through a more common modality such as smartphones remains unattempted.

In its true nature, the properties of air are \emph{contactless} and \emph{ubiquitous}. While intangible, air carries sound, which is propagated as acoustic waves [X]. This basic principle guides our work to explore measuring the rate of airflow through acoustic-based mobile sensing techniques. Let us assume a standard HVAC operations schedule deployed in an office building. It makes its first run of air ventilation early in the morning when the building space is most likely unoccupied. The first ventilation schedule should introduce as much outside air as possible to reduce pollutants accumulated overnight. As the building becomes occupied,, indoor pollutants will increase the need to ventilate again. When an HVAC operation runs, occupants can typically hear ``noise'' coming from the air vent. However, the prominence of us hearing these noises varies with the ambient noise level in the room -- made up of human chatters, appliances, or even outdoor traffic. Indeed, these faint sounds of moving air from the air vents drive our curiosity in using them as a sensing modality; therefore, we seek an understanding in how this noise can be exploited to measure airflow as a data source. 

\subsection{Feasibility}
Broadly speaking, the most basic characteristic of continuously changing audio signals is the frequency range; \emph{low}, \emph{medium}, and \emph{high}. For example, the low-frequency range is between the limits of 10 Hz – 500 Hz \missing{[X]}, common as background noise attributed to the emission from manufactured sources such as computers, vehicles, or even HVAC systems. In actuality, sounds ranging from 20Hz are audible to humans. The mid-range boundary lies between 500Hz to \missing{XXX} Hz, capturing effective communicative sounds from a dog barking to a wide variety of male and female vocals \missing{[X]}. Finally, high-level frequencies range from  \missing{XXX}HZ to \missing{XXX}HZ. These sounds typically consist of musical overtones such as \missing{XXX}, \missing{XXX}, and \missing{XXX} \missing{[X]}. Clearly, the low-frequency audio spectrum is the most relevant to the essence of our research problem. 

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\columnwidth]{final_figures_only/Airflow_spectrums.png}
    \vspace{-4mm}
    \caption{Audio frequency spectrum under different rates of airflow and ambient noises.}
    \label{fig:intuition_spectrum}
\end{figure}

Figure \ref{fig:intuition_spectrum} illustrates the audio frequency spectrum captured within an office space under multiple settings -- an unoccupied room with air ventilation turned on and off, with a variation of expected day-to-day office noises. We can visually inspect that the sound of moving air is approximately below the range of 500 Hz, and the signals remain somewhat consistent over time. 

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.5\linewidth, height=3cm]{final_figures_only/fftbeforeafter.png}
    \vspace{-4mm}
    \caption{XXX - preliminary results show feasibility}
    \label{fig:feasibility}
\end{figure}

To isolate a low-frequency band, we employ a low-pass filter, limiting our cut-off frequency to XXX... range. Ideally, the cut-off frequency for our low-pass filter should guarantee privacy by not detecting any human audible speech. 


% time domain - frequency domain
%range of airflow. % build on previous work

==> backuptext.tex <==
\begin{table} [!h]
\scalebox{.8}{
\centering
  \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\makecell{\textbf{Prediction}}} &
      \multicolumn{4}{c|}{\textbf{Classification}} &
      \multicolumn{2}{c|}{\textbf{Regression}} \\
      & Acc & Prec. & Rec. & F1 & MSE & Reg. \\ \hline
      Vent on/off: 5-fold CV & 0.961 & 0.960 & 0.961 & 0.961 & \cellcolor{black!60} &  \cellcolor{black!60}\\\hline
      Vent on/off: Test & 0.911 & 0.916 & 0.907 & 0.907 & \cellcolor{black!60} & \cellcolor{black!60} \\\Xhline{2\arrayrulewidth}
      Rate of Airflow: 5-fold CV &\cellcolor{black!60} & \cellcolor{black!60} & \cellcolor{black!60} & \cellcolor{black!60} & 0.488 & 0.991 \\\hline
      Rate of Airflow: Test &\cellcolor{black!60} & \cellcolor{black!60} & \cellcolor{black!60} & \cellcolor{black!60} & 3.938 & 0.927 \\\Xhline{2\arrayrulewidth}
  \end{tabular}}
  \caption{Performance comparing train and test of our classification and regression models.}
  \label{tab:smartphone_model}
\end{table}

==> designAlgo.tex <==
\section{Design Algorithm }
\subsection{Acoustic-based ML Model}
1. Classificaiton 
2. Regression
% prediction you foresee

\subsection{Challenges}
\label{sec:challenges}
\subsubsection{Privacy} Figure \ref{X} illustrates the audio frequency spectrum captured within an office space under multiple
settings – an unoccupied room with air ventilation turned on and off, with a variation of expected day-to-day office noises. We can visually inspect that the sound of moving air is approximately below the range of 500 Hz, and the signals remain somewhat consistent over time. As the human speech frequency is overlapping with the airflow spectrum range, we can’t separate the two spectrum simply by filtering. To ensure privacy, if we choose a filter such that it eliminates all human frequencies, then we will be left with very few features for distinguishing airflow. So, there is an important question of how much of these frequencies should we eliminate when preparing audio clips for airflow measurement analysis? To this end, we formulate our first research question: R1: Can we sense airflow using a microphone sensor in a privacy-preserving manner? 
In answering this question, we seek to determine (a) which part of the audio signal spectrum can give us accurate airflow rate estimation? (b) How can we ensure privacy while sensing
airflow? With a privacy-preserved audio spectrum left to analyze, (c) what characteristics of airflow can we accurately sense? 

\subsubsection{Ambient Noise} 
In actuality, low-frequency noise is composed of different day-to-day sources within the environment. One significant challenge is distinguishing noise produced by the HVAC system from other manufactured sources, including office machinery (e.g., photocopier, printer, or moving vehicles), moving vehicles, talking, and other everyday ambient noises (as shown in Figure 1). Accordingly, our second question aims to answer, R2: How robust is our solution in measuring airflow under different levels of ambient noise? 

\subsection{Proposed Techniques}
\label{sec:proposedTech}
\subsubsection{Frequency Domain Filtering}
To isolate a low-frequency band, we can employ a low-pass filter, but must consider the accuracy-privacy trade-off from reducing data dimensionality. From the accuracy perspective, an increased cut-off frequency gives us more feature information to produce better predictions. However, additional frequencies could conceivably interfere with the airflow signal, thus compromising accuracy. Conversely, reducing feature information also results in less features and impact prediction performance. From the privacy perspective, we want the cut-off frequency to be as low as possible to avoid capturing audible noise(especially speech) in the environment. Hence, determining the optimal cut-off frequency for the low-pass filter is essential. We empirically demonstrate how the sound of airflow in audio signals is broadly between 0-500 Hz, thus, limiting our cut-off frequency within this range. We sweep through frequencies in this range and identify the optimal cut-off frequency based on accuracy-privacy trade-off. Ideally, the cut-off frequency for our low-pass filter should guarantee privacy by not detecting any human audible speech.

\subsubsection{Silent Periods}
It is theoretically feasible for our solution to mainly “watch out” for periods where minimal ambient noise is present to measure the rate of airflow as shown in Figure 1 E. By first determining the maximum root mean squared (RMS) noise of air coming from the vent, we can set the RMS noise as a threshold to detect silent periods and collect audio samples for airflow in those periods. While we expect this method to produce the most accurate measure of airflow, prediction capability may fail drastically in loud indoor environments. Also, threshold selection is the major challenge in this approach.

\subsubsection{Minimum Persistent Scheme}
\label{sec:MPS}
We employ this algorithm after getting predictions from the regression model. This algorithm is based on the observation that  airflow signals are continuous and involve minimal fluctuations in pressure that the waves remain relatively constant over a significant period while ambient noise is discrete and varies a lot. Thus, our model overpredicts airflow in the presence of ambient noise. For this reason, we propose MPS that finds minimum persisting airflow value amongst n consecutive predictions. 

we implement a minimum persistence algorithm that takes as input some sequence of continuous samples, of size $n$.  Since we are only interested in the points where ambient noise is not present, we report the minimum non-outlier prediction obtained from the $n$ samples in the sequence.  We introduce two parameters; persistence parameter $p$ and threshold parameter $\epsilon$ which attempt to capture a common minimum value from our model.  Given the sequence of $n$ numbers, we sort the predictions in ascending order, and subsequently attempt to find a "window" of values with size $p$, such that $p$ consecutive values are all within $\pm \epsilon$ of the window's average value.  The algorithm then reports this value as the prediction for all $n$ samples, or, if such a window cannot be found, simply terminates and waits to receive a new batch of $n$ samples.

\begin{wrapfigure}{r}{.6\linewidth}
\centering
\scalebox{.75}{
\begin{minipage}{\linewidth}
\begin{algorithm}[H]
\caption{Minimum Persistent Scheme(MPS) }\label{alg:euclid}
\begin{algorithmic}[1]
\State Initialize $n$, $\epsilon$, $p$

\Procedure{MinimumPersistingValue}{$arr$}\Comment{$arr$ is list of n consecutive predictions}
\State $arr \gets sort(arr)$
\State $per \gets [arr[0]]$ \Comment{initialize the persistence window with the 1st element}
\State $i\gets 1$
\While{$i\not=n$}
\If{$abs(mean(per)-arr[i]) <= \epsilon$}
    \State $per.append(arr[i])$
% \Else
%     \State $y \gets y \times X$
%     \State $N \gets N - 1$
\ElsIf{$abs(mean(per)-arr[i]) > \epsilon$}
    \State $per \gets [arr[i]]$ \Comment{if this element deviates by more than $\epsilon$, start a new window}
% \Else
%     \State $y \gets y \times X$
%     \State $N \gets N - 1$
\EndIf
\If{$length(per) = p$}
    \State return $mean(per)$
\EndIf

\State $i\gets i+1$
\EndWhile
\State return \textbf{failure}
\State
\EndProcedure

% \State $\mu, \sigma = gp.predict(grid)$\Comment{$\mu$ and $\sigma$ are matrices}
% \State \textbf{return} $argmax(\mu + \sigma * \sqrt\beta)$\Comment{UCB aquisition function}

\State $i\gets 0$, $arr[n]$
\While{$i\not=n$}
\State Get $p\_value$\Comment{$p\_value$ is the predicted value given by the model}
\State $arr.append(p\_value)$
\State $i\gets i+1$
\EndWhile

\State MPV = MinimumPersistingValue(arr)
\end{algorithmic}
\end{algorithm}
\end{minipage}%
}
\end{wrapfigure}

==> expEval.tex <==
\section{Experimental Evaluation}
\label{sec:expEval}

We evaluated the experimental setup with Arduino in this section. 

\subsubsection*{Study Procedure}
As shown in Figure \missing{XXX}, we employ the Arduino Nano 33 BLE Sense \missing{[X]} which has an onboard microphone sensor to record sound. Additionally, we utilized the Rev. P wind sensor by Modern Device \missing{[X]}, which is capable of detecting wind direction and speed. The Rev. P wind sensor is solely for collecting ground truth. The wind sensor generates airflow rates in meters per second, which we use as labels for our regression model. We bucketize airflow rates into \emph{1-- on} when the air vent is running, otherwise \emph{0-- off}, for our classification model. Our dataset contains (1-- on: 5000 16ms samples, 0-- off: 5000 16ms samples.) Furthermore, we use a SD card reader module and SD card to store the data files, having features and the corresponding labels.

\subsubsection*{Environment Setup} study takes place in a mid-sized room with a maximum capacity of 6-8 occupants, as a controlled experiment setting. The room is equipped with a de-centralized HVAC unit, and two air vents positioned at two opposite ends of the ceiling room. We use our experimental setup and record data at various locations in the conference room. This includes no air scenario with vent off and different distances and orientations  when the vent is on. All the data is recorded from one vent and in the same room.
%Accordingly, we deployed the two sensors approximately 0.5cm away from each air vent. 
%\textit{Device} - In a commercial implementation, we envision models running locally on devices, as opposed to streaming data to cloud infrastructure as is common today. Edge ML has obvious latency and privacy benefits. For the data recorded from Arduino, we run the ML models on the Laptop. But we also show a case study where the classification and regression models are running locally on different smartphones(Refer to section 6.2.1). The models work in real time on the smartphones with very less prediction time per sample. 

\subsubsection*{Evaluation Metric} 
Accuracy is the most intuitive measure for our classification model, with our dataset being somewhat balanced. We prioritize recall so that our model can accurately predict the air vent running when it is actually turned on. High precision relates to us predicting the air vent switched off when it is not running. F1-score is the weighted average of precision and recall. Next, we utilize the regression score (RS) and mean-squared error (MSE) for our regression model. \missing{Ideally an RS of 0 is.... and MSE of ... explain what you want to achieve}



\subsection{Results}

\subsubsection{Model Selection}


  
\begin{figure}[h]
  \begin{minipage}[h]{.5\linewidth}
    \centering
    \scalebox{.7}{
    \begin{tabular}{|l|c|c|c|c|}\hline
    \toprule
    \textbf{} & \textbf{Acc} & \textbf{Rec} & \textbf{Prec} & \textbf{F1} \\
    \toprule
    Logistic Reg & 0.9810 & [0.9783 0.9834] & [0.9811 0.9809]  & [0.9797 0.9821 ]\\ \hline
    SVC & 0.9851 & [0.9812 0.9885] & [0.9869 0.9835] & [0.9840 0.9860]\\ \hline
    KNN & 0.9884 & [0.9769 0.9987] & [0.9985 0.98] & [0.9876 0.9893] \\ \hline
    DT & 0.9858 & [0.9740 0.9962] & [0.9955 0.9775    ] & [0.9846 0.9867] \\ \hline
    XGBoost & 0.9912 & [0.9826 0.9987] & [0.9985 0.9849] & [0.9905 0.9917] \\\hline
    \end{tabular}} 
    \caption{Performance comparison of different Classification ML models}
    \label{tab:ml}
  \end{minipage}\hfill
  \begin{minipage}[h]{.5\linewidth}
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/ML_models.png}
    \caption{Performance comparison of different Regression ML models}
    \label{fig:ml}
  \end{minipage}
\end{figure}



We need to select the ML model for a) regression: predicting rate of airflow and b) classification: classifying vent status. We identify commonly used classification models and regression models and train all of them. For the classification model, we compare the accuracy, precision and recall of the classification models trained. For the regression model, we compare regression scores of different models. For simplicity, we fix the cut-off frequency to 375 Hz in all the cases. 



The results are shown in figure \ref{fig:ml}. 
It can be clearly seen that the linear model does not perform well in classification or regression. This means that our data is non-linear. One approach that we can try is basis expansion to classify or predict non-linear data. But in this case we don't have any idea of how the distribution looks like. Since there are 7 features, we can't plot and observe the distribution empirically. 
Now, we try other ML models. Out of other models, Decision trees and Gradient boosting models perform really well on the given data. We choose gradient boosting model over decision trees as its accuracy is slightly more than decision trees and it has other added advantages of low complexity. Thus, it can easily run on edge devices in real time.

The overall accuracy of the classification and regression models are: 
\begin{figure}[H]
\begin{minipage}[h]{.4\linewidth}
\centering
%\scalebox{0.7}{
\begin{tabular}{|l|c|c|}\hline
\textbf{Regression } & \textbf{Mean Sq. Err.} & \textbf{Reg Score}\\ \hline
Training Data  & 0.07 & 0.99\\ \hline
Test Data  & 4.12 & 0.95 \\ \hline
\end{tabular}%} 
\caption{Regression performance, quantified with mean squared error and regression score, of \names regression model for train and test datasets.}
\label{tab:regmodelgenresults}
\end{minipage}\hfill
\begin{minipage}[h]{.55\linewidth}
\centering
%\scalebox{0.7}{
\begin{tabular}{|l|c|c|c|c|}\hline
\textbf{Classification} & \textbf{Acc.} & \textbf{Rec.} & \textbf{Pr.} & \textbf{F1}\\ \hline
Training Data  & 0.9941 & [0.9897 0.9977] & [0.9974 0.9912] & [0.9935 0.9944] \\ \hline
Test Data  & 0.9912 & [0.9826 0.9987] & [0.9985 0.9849] & [0.9905 0.9917] \\ \hline
\end{tabular}%} 
\caption{Classification performance, quantified with accuracy, precision, recall, and F1 score for \names classification model on training and test data.}
\label{tab:arduino_models}
\end{minipage}
\end{figure}

These results show that the proposed system can classify the vent status with very high accuracy of 99\% and estimate the rate of airflow with an accuracy of 95\%. 



\subsubsection{Model Generalization on Types of Vents}

Previous experiment was a model trained and tested on the same vent. In this section, we seek to determine if the model can be generalized to different vents, either located in a different room/building or different vent-type (ceiling/side). For this, we record test data of 20 minutes from different vents and run the trained model on it. 
\ref{tab:vents} shows the results of this experiment. The key observation here is that the vents that have similar geometry does not require retraining. But the vents of different type or having different geometry will require retraining. 



\begin{figure}[h]
 
    \centering
    \scalebox{1}{
    \begin{tabular}{|c|c|c|c|}
    \hline
        Vent  & Type & Location & Test MSE  \\ \hline
       v1  & Ceiling Vent & A313C conference room & 1.61\\ \hline
       v2 & Ceiling Vent & A313C conference room & 1.78\\ \hline
       v3 & Ceiling Vent & A331 LASS  & 1.92\\ \hline
       v4 & Ceiling Vent & CICS building & 1.84\\ \hline
       v5 & Ceiling Vent(different type) & Home vent  & 5.29\\ \hline
       v6 & Side vent & A313B  & 22.69\\ \hline
    \end{tabular}} 
    \caption{Performance of regression models for different vents}
    \label{tab:vents}

\end{figure}



\subsubsection{Selecting the Cut-off Frequency}


The selection of ideal cut-off frequency that maintains the trade-off between accuracy and privacy of the system is very crucial. First, we empirically observe the airflow signal spectrum and found that it ranges roughly between 0-500Hz. So, we sweep through all the candidate frequencies(based on FFT bin size) in this range and train the model with that cut-off frequency. This was we trained 8 different models using different cut-off frequencies and kept other parameters constant. Then, we observe the train and test MSE for each model. The results are shown in Figure \ref{fig:cutoffFreq}

As expected the test MSE when cut-off frequency is less that 250 Hz is very high. This is because there are not enough features for the model to learn. After this, the test MSE reduces to a minimum value. But when cut-off frequency increases above 375 Hz, the test MSE begins to rise as the audible frequencies starts becoming dominant which leads to incorrect predictions. 


\begin{figure}
    \centering
    \centering
    \includegraphics[width=0.5\columnwidth]{figures/cut_off.png}
    \caption{Determining Ideal Cut-off Frequency in classification}
    \label{fig:cutoffFreq}
\end{figure}

\subsubsection{Privacy Evaluation}
There are numerous privacy concerns surrounding always-on microphones in our homes placed in locations where they have access to private conversation. We
performed a user study, evaluating whether our participants were
able to perceive various levels of content within a series of audio
clips, as if they were an eavesdropper listening to a \names audio stream.

\textbf{Procedure}
We generated 4 audio files file A original, file A filtered, file B original, and file B filtered from Wikipedia, each of 30 seconds duration. The file A original and file B original are two different files recorded by different people from Wikipedia, and file A filtered and file B filtered are the files resulting after passing the original files through \name. Thus, the filtered(cut-off 375 Hz) files are low pass filtered versions of original files. All files were saved as WAV files. \\We conducted a user study with 12 participants (6 male, 5 female and 1 non-binary) between ages 20-34 (mean 25.1) and asked them, for each file, to respond a set of questions on a scale of 1 to 5 as shown in Table 2. This study is IRB approved. The participation begins with turning in a signed copy of this consent form. Each participant is issued a random 2 character identifier. Accordingly, the investigator conducts a 5 minutes walkthrough of the study materials used in this study. Specifically, the investigator explains the survey that needs to fill up upon hearing a set of audio recordings. During the main study, participants are handed a laptop preloaded with a list of audio clips and a headset to hear these recordings. The default volume set on the laptop will be at 50\%. However, participants have the option of lowering/increasing the volume based on their preference. Once they are comfortable with the settings, they start listening to one recording at a time lasting for 30 seconds. Then they turn to the survey and rate the audibility of human speech in the clip you just listened to. This process repeats until all the audio clips have been heard and evaluated. This process did not take more than 3 minutes per participant. 

\textbf{Results}
For file A original and file B original, the participants were able to clearly hear and discern speech well enough to transcribe. All the participants correctly identified the speech in these files. For file A original, they wrote comments like "talking about water flow", "movement of water in the ocean", "Movement of water masses", etc. For file B original, they wrote comments like "discussion of airflow and pressure", "measurement of airflow, air pressure, molecules", "airflow and air pressure", etc. However, for the filtered files, participants were able to hear something, but could not say for sure that it was human speech and could not discern it at all.

For file A filtered, they wrote comments like "random noises", "garbled sounds, white noise", "Mostly noisy", etc.

For file B filtered, they wrote "noise again", "white noise", etc


\textbf{NLP Results}
Additionally, we processed our audio files through various natural
language processing service (Google Speech Recognition) and found it was
able to detect speech content within the filtered files. While it was able to transcribe the original, unfiltered audio file correctly.


\begin{table} [!h]
\scalebox{0.8}{
\centering
  \begin{tabular}{|l|c|c|c|c|}
    \hline
    \multirow{2}{*}{\makecell{\textbf{Questionnaire}}} &
      \multicolumn{2}{c|}{\textbf{File A}} &
      \multicolumn{2}{c|}{\textbf{File B}} \\
      & Original & Filtered & Original & Filtered \\ \hline
      Were you able to hear anything in the file? & M=5.00,SD=0.00 & M=1.83,SD=1.52 & M=5.00,SD=0.00 & M=2.17,SD=1.47 \\ \hline
      
      \makecell[l]{Were you able to hear human sounds in the file? \\(i.e., sounds that could be coming from a human)} &M=5.00,SD=0.00  &  M=1.67,SD=0.39& M=5.00,SD=0.00 & M=2.08,SD=0.99 \\\hline
      
      \makecell[l]{Were you able to hear any speech in the file?} & M=4.83,SD=0.58 & M=1.16,SD=0.39& M=5.00,SD=0.00 & M=1.75,SD=1.05\\\hline
      
      \makecell[l]{Were you able to discern speech well enough to transcribe?} & M=4.75,SD=0.45 & M=1.00,SD=0.00 & M=4.92,SD=0.29 & M=1.08,SD=0.29\\\hline
      
      \makecell[l]{General comments: What did you hear if at all,\\what you perceived was in the file, can you transcribe?} & & & & \\\hline
      
      What is your age? & \multicolumn{4}{l|}{M=25.09,SD= 4.72} \\\hline
      
      What gender do you identify as? & \multicolumn{4}{l|}{M:6, F:5, NB: 1} \\\hline

      What is your level of education? & \multicolumn{4}{l|}{7 Graduate} \\\hline
      
  \end{tabular}}
  \caption{Summary statistics of privacy evaluation questionnaire.}
  \label{tab:my_label}
\end{table}


The richness of sound is a double-edged sword. On one hand, it enables fine grained activity sensing, while also capturing
potentially sensitive audio, including spoken content. This is an inherent and unavoidable danger of using microphones as sensors. However, we note that always-listening devices –especially smartphones and smart speakers – are becoming more prevalent and accepted in homes and workplaces, and
so the social stigma of such devices may wane in the coming years.  Moreover,
we envision our model being run locally on devices (as we showed possible with smartphone ), such that audio data never has to be transmitted. Furthermore, we also employ silent--period detection in the prepossessing module which further guarantees the privacy of the proposed system.


\subsection{Summary of findings}

Through the feasibility studies, we observe that Gradient boosting outperforms other commonly used ML models for predicting rate of airflow in terms of accuracy and model complexity. Using this model, the proposed system can accurately classify the vent status and determine the rate of airflow. The proposed system can be easily generalized to different vents having the same geometry. But, if the vent geometry is different, it will require retraining the system. We also show that 375 Hz is the optimal cut-off frequency of the low pass filter to have enough features for the models to learn airflow characteristics. Through an extensive user study, we further show that the user privacy is ensured if we use 375 Hz low pass filtered audio files. While all these experiments are done in very low ambient noise environments, in the next section, we explore the performance of this system in high ambient noise scenarios. 

==> feasibility.tex <==
\section{Feasibility Study}
\label{sec:feasibility}
We conduct a feasibility study to understand how a microphone sensor can detect airflow changes over time. 

\subsubsection*{Study Procedure}
As shown in Figure \missing{XXX}, we employ the Arduino Nano 33 BLE Sense \missing{[X]} which has an onboard microphone sensor to record sound. Additionally, we utilized the Rev. P wind sensor by Modern Device \missing{[X]}, which is capable of detecting wind direction and speed. The Rev. P wind sensor is solely for collecting ground truth. The wind sensor generates airflow rates in meters per second, which we use as labels for our regression model. We bucketize airflow rates into \emph{1-- on} when the air vent is running, otherwise \emph{0-- off}, for our classification model. Our dataset contains (1-- on: 5000 16ms samples, 0-- off: 5000 16ms samples.) Furthermore, we use a SD card reader module and SD card to store the data files, having features and the corresponding labels.

\subsubsection*{Environment Setup} study takes place in a mid-sized room with a maximum capacity of 6-8 occupants, as a controlled experiment setting. The room is equipped with a de-centralized HVAC unit, and two air vents positioned at two opposite ends of the ceiling room. We use our experimental setup and record data at various locations in the conference room. This includes no air scenario with vent off and different distances and orientations  when the vent is on. All the data is recorded from one vent and in the same room.
%Accordingly, we deployed the two sensors approximately 0.5cm away from each air vent. 
%\textit{Device} - In a commercial implementation, we envision models running locally on devices, as opposed to streaming data to cloud infrastructure as is common today. Edge ML has obvious latency and privacy benefits. For the data recorded from Arduino, we run the ML models on the Laptop. But we also show a case study where the classification and regression models are running locally on different smartphones(Refer to section 6.2.1). The models work in real time on the smartphones with very less prediction time per sample. 

\subsubsection*{Evaluation Metric} 
Accuracy is the most intuitive measure for our classification model, with our dataset being somewhat balanced. We prioritize recall so that our model can accurately predict the air vent running when it is actually turned on. High precision relates to us predicting the air vent switched off when it is not running. F1-score is the weighted average of precision and recall. Next, we utilize the regression score (RS) and mean-squared error (MSE) for our regression model. \missing{Ideally an RS of 0 is.... and MSE of ... explain what you want to achieve}



\subsection{Results}

\subsubsection{Model Selection}


  
\begin{figure}[h]
  \begin{minipage}[h]{.5\linewidth}
    \centering
    \scalebox{.7}{
    \begin{tabular}{|l|c|c|c|c|}\hline
    \toprule
    \textbf{} & \textbf{Acc} & \textbf{Rec} & \textbf{Prec} & \textbf{F1} \\
    \toprule
    Logistic Reg & 0.9810 & [0.9783 0.9834] & [0.9811 0.9809]  & [0.9797 0.9821 ]\\ \hline
    SVC & 0.9851 & [0.9812 0.9885] & [0.9869 0.9835] & [0.9840 0.9860]\\ \hline
    KNN & 0.9884 & [0.9769 0.9987] & [0.9985 0.98] & [0.9876 0.9893] \\ \hline
    DT & 0.9858 & [0.9740 0.9962] & [0.9955 0.9775    ] & [0.9846 0.9867] \\ \hline
    XGBoost & 0.9912 & [0.9826 0.9987] & [0.9985 0.9849] & [0.9905 0.9917] \\\hline
    \end{tabular}} 
    \caption{Performance comparison of different Classification ML models}
    \label{tab:ml}
  \end{minipage}\hfill
  \begin{minipage}[h]{.5\linewidth}
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/ML_models.png}
    \caption{Performance comparison of different Regression ML models}
    \label{fig:ml}
  \end{minipage}
\end{figure}



We need to select the ML model for a) regression: predicting rate of airflow and b) classification: classifying vent status. We identify commonly used classification models and regression models and train all of them. For the classification model, we compare the accuracy, precision and recall of the classification models trained. For the regression model, we compare regression scores of different models. For simplicity, we fix the cut-off frequency to 375 Hz in all the cases. 



The results are shown in figure \ref{fig:ml}. 
It can be clearly seen that the linear model does not perform well in classification or regression. This means that our data is non-linear. One approach that we can try is basis expansion to classify or predict non-linear data. But in this case we don't have any idea of how the distribution looks like. Since there are 7 features, we can't plot and observe the distribution empirically. 
Now, we try other ML models. Out of other models, Decision trees and Gradient boosting models perform really well on the given data. We choose gradient boosting model over decision trees as its accuracy is slightly more than decision trees and it has other added advantages of low complexity. Thus, it can easily run on edge devices in real time.

The overall accuracy of the classification and regression models are: 
\begin{figure}[H]
\begin{minipage}[h]{.4\linewidth}
\centering
%\scalebox{0.7}{
\begin{tabular}{|l|c|c|}\hline
\textbf{Regression } & \textbf{Mean Sq. Err.} & \textbf{Reg Score}\\ \hline
Training Data  & 0.07 & 0.99\\ \hline
Test Data  & 4.12 & 0.95 \\ \hline
\end{tabular}%} 
\caption{Regression performance, quantified with mean squared error and regression score, of \names regression model for train and test datasets.}
\label{tab:regmodelgenresults}
\end{minipage}\hfill
\begin{minipage}[h]{.55\linewidth}
\centering
%\scalebox{0.7}{
\begin{tabular}{|l|c|c|c|c|}\hline
\textbf{Classification} & \textbf{Acc.} & \textbf{Rec.} & \textbf{Pr.} & \textbf{F1}\\ \hline
Training Data  & 0.9941 & [0.9897 0.9977] & [0.9974 0.9912] & [0.9935 0.9944] \\ \hline
Test Data  & 0.9912 & [0.9826 0.9987] & [0.9985 0.9849] & [0.9905 0.9917] \\ \hline
\end{tabular}%} 
\caption{Classification performance, quantified with accuracy, precision, recall, and F1 score for \names classification model on training and test data.}
\label{tab:arduino_models}
\end{minipage}
\end{figure}

These results show that the proposed system can classify the vent status with very high accuracy of 99\% and estimate the rate of airflow with an accuracy of 95\%. 


\subsubsection{Baseline Real World Setup: Accuracy of Classifying Vent Status and Rate of Air Flow}
\begin{enumerate}
    \item This will be our baseline results, in that, using an arduino microphone setup, positioned as close as 0.5m and as far as 2.5m away from the vent will give us the following performance in a small conference room. See Table \ref{tab:realworld}
    \item Hence, results here are based on experimental setup above to depict real-world deployment
    \item start off with experimenting on distance of arduino microphone from the air supply vent
    \item with optimal distance from (2), test performance of model on experimental setup under two conditions, \emph{unoccupied} or \emph{occupied - 3 actual people in the room} at closest distance (0.5m) and furthest distance (2.5m) 
\end{enumerate}

\begin{table}[h!]
    \centering
    \scalebox{.7}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|}\hline
    \toprule
    \textbf{Experiment Setup} & \textbf{Acc} & \textbf{Prec} & \textbf{Rec} & \textbf{Train Train MSE} & \textbf{Train Reg Score} & \textbf{Test MSE} & \textbf{Test Reg Score} \\
    \toprule
    \textbf{Unoccupied} with arduino at \textbf{0.5m} away from vent & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
    \textbf{Occupied} with arduino at \textbf{0.5m} away from vent  & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
    \textbf{Unoccupied} with arduino at \textbf{2.5m} away from vent & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
    \textbf{Occupied} with arduino at \textbf{2.5m} away from vent & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\\hline
    \end{tabular}} 
    \caption{Real world performance of classification and regression models}
    \label{tab:realworld}
\end{table}

\subsubsection{Model Generalization on Types of Vents}

Previous experiment was a model trained and tested on the same vent. In this section, we seek to determine if the model can be generalized to different vents, either located in a different room/building or different vent-type (ceiling/side). For this, we record test data of 20 minutes from different vents and run the trained model on it. 
\ref{tab:vents} shows the results of this experiment. The key observation here is that the vents that have similar geometry does not require retraining. But the vents of different type or having different geometry will require retraining. 

% Accordingly, we also experiment with model personalization to see if it improves accuracy. 
% data is collected from 5 vents.
% In a generalized case, model is trained on 4 vents and tested on 1 vent. We repeat this experiment for all 5 vents and report the average performance.
% In a personalized cased, model is trained on 4 vents and 30\% data from 1 test vent. It is then tested on 70\% data from 1 test vent. We repeat this experiment for all 5 vents and report the average performance.
% In the regression plot, we chart the rate of airflow from all 5 vents predicted using generalized and personalized model.


\begin{figure}[h]
 
    \centering
    \scalebox{1}{
    \begin{tabular}{|c|c|c|c|}
    \hline
        Vent  & Type & Location & Test MSE  \\ \hline
       v1  & Ceiling Vent & A313C conference room & 1.61\\ \hline
       v2 & Ceiling Vent & A313C conference room & 1.78\\ \hline
       v3 & Ceiling Vent & A331 LASS  & 1.92\\ \hline
       v4 & Ceiling Vent & CICS building & 1.84\\ \hline
       v5 & Ceiling Vent(different type) & Home vent  & 5.29\\ \hline
       v6 & Side vent & A313B  & 22.69\\ \hline
    \end{tabular}} 
    \caption{Performance of regression models for different vents}
    \label{tab:vents}

\end{figure}


% \begin{figure}[h]
%   \begin{minipage}[h]{.45\linewidth}
%     \centering
%     \scalebox{1}{
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%          & Accuracy & Precision & Recall \\ \hline
%       Generalized  &  & &\\ \hline
%       Personalized &  & &\\ \hline
%     \end{tabular}} 
%     \caption{Performance of generalized and personalized classification models for different vents}
%     \label{tab:my_label}
%   \end{minipage}\hfill
%   \begin{minipage}[h]{.5\linewidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/ventTypeRegressionFeasibility_placeholder.jpg}
%     \caption{Performance of generalized and personalized regression models for different vents}
%     \label{fig:ml}
%   \end{minipage}
% \end{figure}


\subsubsection{Selecting the Cut-off Frequency}


The selection of ideal cut-off frequency that maintains the trade-off between accuracy and privacy of the system is very crucial. First, we empirically observe the airflow signal spectrum and found that it ranges roughly between 0-500Hz. So, we sweep through all the candidate frequencies(based on FFT bin size) in this range and train the model with that cut-off frequency. This was we trained 8 different models using different cut-off frequencies and kept other parameters constant. Then, we observe the train and test MSE for each model. The results are shown in Figure \ref{fig:cutoffFreq}

As expected the test MSE when cut-off frequency is less that 250 Hz is very high. This is because there are not enough features for the model to learn. After this, the test MSE reduces to a minimum value. But when cut-off frequency increases above 375 Hz, the test MSE begins to rise as the audible frequencies starts becoming dominant which leads to incorrect predictions. 


\begin{figure}
    \centering
    \centering
    \includegraphics[width=0.5\columnwidth]{figures/cut_off.png}
    \caption{Determining Ideal Cut-off Frequency in classification}
    \label{fig:cutoffFreq}
\end{figure}

\subsubsection{Privacy Evaluation}
There are numerous privacy concerns surrounding always-on microphones in our homes placed in locations where they have access to private conversation. We
performed a user study, evaluating whether our participants were
able to perceive various levels of content within a series of audio
clips, as if they were an eavesdropper listening to a \names audio stream.

\textbf{Procedure}
We generated 4 audio files file A original, file A filtered, file B original, and file B filtered from Wikipedia, each of 30 seconds duration. The file A original and file B original are two different files recorded by different people from Wikipedia, and file A filtered and file B filtered are the files resulting after passing the original files through \names. Thus, the filtered(cut-off 375 Hz) files are low pass filtered versions of original files. All files were saved as WAV files. \\We conducted a user study with 12 participants (6 male, 5 female and 1 non-binary) between ages 20-34 (mean 25.1) and asked them, for each file, to respond a set of questions on a scale of 1 to 5 as shown in Table 2. This study is IRB approved. The participation begins with turning in a signed copy of this consent form. Each participant is issued a random 2 character identifier. Accordingly, the investigator conducts a 5 minutes walkthrough of the study materials used in this study. Specifically, the investigator explains the survey that needs to fill up upon hearing a set of audio recordings. During the main study, participants are handed a laptop preloaded with a list of audio clips and a headset to hear these recordings. The default volume set on the laptop will be at 50\%. However, participants have the option of lowering/increasing the volume based on their preference. Once they are comfortable with the settings, they start listening to one recording at a time lasting for 30 seconds. Then they turn to the survey and rate the audibility of human speech in the clip you just listened to. This process repeats until all the audio clips have been heard and evaluated. This process did not take more than 3 minutes per participant. 

\textbf{Results}
For file A original and file B original, the participants were able to clearly hear and discern speech well enough to transcribe. All the participants correctly identified the speech in these files. For file A original, they wrote comments like "talking about water flow", "movement of water in the ocean", "Movement of water masses", etc. For file B original, they wrote comments like "discussion of airflow and pressure", "measurement of airflow, air pressure, molecules", "airflow and air pressure", etc. However, for the filtered files, participants were able to hear something, but could not say for sure that it was human speech and could not discern it at all.

For file A filtered, they wrote comments like "random noises", "garbled sounds, white noise", "Mostly noisy", etc.

For file B filtered, they wrote "noise again", "white noise", etc


\textbf{NLP Results}
Additionally, we processed our audio files through various natural
language processing service (Google Speech Recognition) and found it was
able to detect speech content within the filtered files. While it was able to transcribe the original, unfiltered audio file correctly.

% Plan to evaluate:\\
% - read 1-min text from Wikipedia\\
% - run through privacy algo and have participants to evaluate audibility of processed audio clip.\\
% - coupled with NLP results using Google Speech Recognition
\begin{table} [!h]
\scalebox{0.8}{
\centering
  \begin{tabular}{|l|c|c|c|c|}
    \hline
    \multirow{2}{*}{\makecell{\textbf{Questionnaire}}} &
      \multicolumn{2}{c|}{\textbf{File A}} &
      \multicolumn{2}{c|}{\textbf{File B}} \\
      & Original & Filtered & Original & Filtered \\ \hline
      Were you able to hear anything in the file? & M=5.00,SD=0.00 & M=1.83,SD=1.52 & M=5.00,SD=0.00 & M=2.17,SD=1.47 \\ \hline
      
      \makecell[l]{Were you able to hear human sounds in the file? \\(i.e., sounds that could be coming from a human)} &M=5.00,SD=0.00  &  M=1.67,SD=0.39& M=5.00,SD=0.00 & M=2.08,SD=0.99 \\\hline
      
      \makecell[l]{Were you able to hear any speech in the file?} & M=4.83,SD=0.58 & M=1.16,SD=0.39& M=5.00,SD=0.00 & M=1.75,SD=1.05\\\hline
      
      \makecell[l]{Were you able to discern speech well enough to transcribe?} & M=4.75,SD=0.45 & M=1.00,SD=0.00 & M=4.92,SD=0.29 & M=1.08,SD=0.29\\\hline
      
      \makecell[l]{General comments: What did you hear if at all,\\what you perceived was in the file, can you transcribe?} & & & & \\\hline
      
      What is your age? & \multicolumn{4}{l|}{M=25.09,SD= 4.72} \\\hline
      
      What gender do you identify as? & \multicolumn{4}{l|}{M:6, F:5, NB: 1} \\\hline

      What is your level of education? & \multicolumn{4}{l|}{7 Graduate} \\\hline
      
  \end{tabular}}
  \caption{Summary statistics of privacy evaluation questionnaire.}
  \label{tab:my_label}
\end{table}

% We continuously observed the frequency spectrum of the microphone signal over one day where two conditions can be expected; the HVAC unit is turned on or off. %with and without air?
% Subsequently, we sought to infer about the plausibility of using microphone signals distinguish a) \emph{when the ventilation system is turned on/off} and b) \emph{the rate of airflow within the enclosed space}. 

The richness of sound is a double-edged sword. On one hand, it enables fine grained activity sensing, while also capturing
potentially sensitive audio, including spoken content. This is an inherent and unavoidable danger of using microphones as sensors. However, we note that always-listening devices –especially smartphones and smart speakers – are becoming more prevalent and accepted in homes and workplaces, and
so the social stigma of such devices may wane in the coming years.  Moreover,
we envision our model being run locally on devices (as we showed possible with smartphone ), such that audio data never has to be transmitted. Furthermore, we also employ silent--period detection in the prepossessing module which further guarantees the privacy of the proposed system.

% In addressing (a), \ncz{How should I be justifying this? Graph? How to quantify significance?} \missing{There is a significant difference between these two spectograms. Due to this, the classification model that classifies the presence of air has 100\% accuracy.}



% To establish that the proposed system is capable of estimating the rate of airflow and not just its presence, we observe the spectogram of the low pass filtered microphone signal for the following cases
% \begin{itemize}
%     \item Different rates of airflow at a fixed distance
%     \item Fixed rate of airflow at different distance.
% \end{itemize}


\subsection{Summary of findings}

Through the feasibility studies, we observe that Gradient boosting outperforms other commonly used ML models for predicting rate of airflow in terms of accuracy and model complexity. Using this model, the proposed system can accurately classify the vent status and determine the rate of airflow. The proposed system can be easily generalized to different vents having the same geometry. But, if the vent geometry is different, it will require retraining the system. We also show that 375 Hz is the optimal cut-off frequency of the low pass filter to have enough features for the models to learn airflow characteristics. Through an extensive user study, we further show that the user privacy is ensured if we use 375 Hz low pass filtered audio files. While all these experiments are done in very low ambient noise environments, in the next section, we explore the performance of this system in high ambient noise scenarios. 

==> feasibility_old.tex <==
\section{Feasibility Study}
To assess the practicality of our proposed system, we conduct a feasibility study to understand how a microphone sensor would detect the change in air pressure over time. 

\subsection{Experimental Setup}
Figure \ref{fig:arduino_setup} shows our experimental setup for the study. Specifically, we employed the Arduino Nano 33 BLE Sense \todo{[XXX]} which has an onboard microphone sensor to record sound. Additionally, we utilized the Rev. P wind sensor by Modern Device \todo{[XXX]}, which is capable of detecting wind direction and speed. The Rev. P wind sensor is solely for collecting ground truth. 

\ncz{You need to describe the environmental too. I had written this, please correct the details.} \todo{The experiments were conducted in a mid-sized conference room with a maximum capacity of 6-8 occupants. The room is equipped with a de-centralized HVAC unit, and two air vents positioned at two opposite ends of the ceiling room. Accordingly, we deployed the two sensors approximately 1 ft away from the air vent. For this experiment, the room remained unoccupied. In what follows, we present the results of our experiments, conducted over one day.}

\subsection{Results}
\subsubsection{Accuracy of Regression and Classification Models}
Validation in real world
-pick one setup 
\subsubsection{Rate of Airflow}

How we are planning to show this is by testing model on different airflow sources, 2 fans and 1 air purifier. 
- exact rate of airflow
- bucketizing rate of airflow into low medium high. due to this, we cannot account for building vents.

- perform experiments for vent only, bucketising 

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{air1.png}
         \caption{Low Airflow}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{air2.png}
         \caption{Medium Airflow}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{air3.png}
         \caption{High Airflow}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Spectrum of low pass filtered microphone signal with different rates of airflow at a fixed distance of 1m}
        \label{fig:three graphs}
\end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.5\columnwidth]{Combined_CDF_flow.jpg}
    \caption{CDF for different rates of airflow at fixed distance}
    \vspace{-4mm}
    \label{fig:concept}
\end{figure}

\subsubsection{Distance of Microphone}


- add table of distance 0 - 2.5m on arduino 

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
          distance(m) & 0.5 & 1 & 1.5 & 2.25 \\ \hline
          Test MSE & 2.0555 & 1.7999 & 0.8428 & 1.6951 \\ \hline
    \end{tabular}
    \caption{Accuracy of regression model at different distances}
    \label{tab:my_label}
\end{table}



\subsubsection{Type of Buildings}

\begin{table}[]
    \centering
    
    \begin{tabular}{|c|c|c|}
    \hline
      Vent  & Environment & Test MSE \\ \hline
      Ceiling Vent 1   &  Conference room A313C (4mX2mX3m) & 1.6087 \\ \hline
      Ceiling Vent 2
(same type as vent 1)   &  Conference room A313C (4mX2mX3m) & 1.4046

 \\ \hline
     Ceiling  Vent 3(same type as vent 1)   &  CICS & 1.8450
\\ \hline
       Vent 4   &  Side vent A313A
 & 22.698 \\ \hline
 
       Ceiling Vent 5  & Home
 & 24.8025
 \\ \hline
 
        Vent 6 (Fan)  &  Home 
 & 17.2671 \\ \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
- need to re-run with 250Hz model

\subsubsection{Privacy}

Plan to evaluate:
- read 1-min text from Wikipedia
- run through privacy algo and have participants to evaluate audibility of processed audio clip.
- coupled with NLP results using Google Speech Recognition


We continuously observed the frequency spectrum of the microphone signal over one day where two conditions can be expected; the HVAC unit is turned on or off. %with and without air?
Subsequently, we sought to infer about the plausibility of using microphone signals distinguish a) \emph{when the ventilation system is turned on/off} and b) \emph{the rate of airflow within the enclosed space}. 

The richness of sound is a double-edged sword. On one hand,
it enables fine grained activity sensing, while also capturing
potentially sensitive audio, including spoken content. This is
an inherent and unavoidable danger of using microphones as
sensors. However, we note that always-listening devices –
especially smartphones and smart speakers – are becoming
more prevalent and accepted in homes and workplaces, and
so the social stigma of such devices may wane in the coming
years. 
Moreover,
we envision our model being run locally on devices (as we
showed possible with smartphone ), such that audio data never has to be transmitted. 

In addressing (a), \ncz{How should I be justifying this? Graph? How to quantify significance?} \todo{There is a significant difference between these two spectograms. Due to this, the classification model that classifies the presence of air has 100\% accuracy.}

\begin{figure}
    \centering
    \includegraphics[width=90mm]{experimental_setup.png}
    \caption{Experimental Setup. \todo{another photo on the side where we can show where it is fixed.}}
    \label{fig:arduino_setup}
\end{figure}

To establish that the proposed system is capable of estimating the rate of airflow and not just its presence, we observe the spectogram of the low pass filtered microphone signal for the following cases
\begin{itemize}
    \item Different rates of airflow at a fixed distance
    \item Fixed rate of airflow at different distance.
\end{itemize}

Fig. 2 shows the spectrum of microphone signal with different rates of airflow. It can be observed that with the increase in rate of airflow, the amplitude at low frequency components increase. 

Fig. 3 shows the spectrum of microphone signal at different distances . It is clear from that figure that with increase in distance, the amplitude at low frequency components decrease. This is because the air experienced decreases with increase in distance. However, this change is not linear.

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{air1.png}
         \caption{Low Airflow}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{air2.png}
         \caption{Medium Airflow}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{air3.png}
         \caption{High Airflow}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Spectrum of low pass filtered microphone signal with different rates of airflow at a fixed distance of 1m}
        \label{fig:three graphs}
\end{figure}

To understand these graphs in detail, we plot the CDF of these graphs as shown in Figure. \\
\textbf{Insight: }The CDF shows that as the rate of airflow increases, the CDF becomes smoother and steeper. 





\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{air2_1m.png}
         \caption{1 m}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{air2_1_5m.png}
         \caption{1.5 m }
         \label{fig:five over x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{air2_2_25m.png}
         \caption{2.25 m}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Spectrum of low pass filtered microphone signal with fixed rates of airflow at different distances.}
        \label{fig:three more graphs}
\end{figure}

To understand these graphs in detail, we plot the CDF of these graphs as shown in Figure. \\
\textbf{Insight: }The CDF shows that as the distance increases, the less frequencies are involved. For example: at 50cm, the slope is till 300 or so. While at 1.5 m, the slope is till 200.



\begin{figure}[ht!]
    \centering
    \includegraphics[width=\columnwidth]{Combined_CDF_dist.jpg}
    \caption{CDF for different distances at fixed rate of airflow}
    \vspace{-4mm}
    \label{fig:concept}
\end{figure}

==> implementation.tex <==
\section{\names Implementation}
\label{sec:implementation}
%we show smartphone and arduino pipeline, change feature extractor ot FFT,define two experimental setup
In this section, we implement our proposed system, \name. Figure \ref{fig:sysOverview} illustrates our experimental setup using two input sources, (1) an Arduino Nano BLE Sense and (2) Smartphone microphone, predicting two airflow characteristics, namely, the state of air vents and the rate of airflow. Note that our project consisting of datasets, models, and visualizations are available for researchers alike. These resources can be accessed through: [link redacted].

\begin{figure}[!h]
\centering
    \includegraphics[width=\linewidth]{final_figures_only/system.jpg}
    \caption{System overview of \name, consisting of three components.}
    \label{fig:sysOverview}
\end{figure}

We implement \names using \emph{scikit-learn} Python framework, and \emph{Noise} wrapper for \emph{kissfft} FFT computation library \cite{noise,kissfft}. We also utilize the \emph{JPMML} project to convert our Python-trained model into a Java-compatible object, allowing the computation of predictions directly on the smartphone \cite{jpmml}.
 
\subsubsection*{Context Awareness Module}
Our smartphone application extends a context awareness module, which senses device movement, orientation, and phone exposure. We will later explain in Section \ref{sec:devicepos} how \names best operates when the microphone lies unobstructed and faces towards the HVAC air vent. Thus, this module infers phone exposure using proximity and light sensor APIs, accessible through the SensorManager framework. Phone movement and orientation use standard accelerometer API.

\subsubsection*{Sampling and Filtering}
\names captures audio signals from the microphone at 16 kHz. We based this decision on our review of smartphone specifications, where the lowest standard native sampling frequency across modern Android and iOS phones is 16 kHz. The primary function of our filtering module is ensuring user privacy and remove high frequencies and ambient noise from the signal. We achieve this goal in several steps: First, the module divides the audio signal into segments of $n$ ms. Second, it employs a two-step filtering method to primarily preserve user-privacy, (1) it runs a silent-period detection algorithm, which iteratively discards audio clips that contain audible human speech and (2) it applies a low pass filter to remove high frequency ambient noises, including residual fragments of human voices during the silent periods. As we will discuss in Section \ref{sec:expEval}, our experiments found the optimal cut-off frequency of the low pass filter at 375 Hz.
%Note, however, that the clips it continues to process may still contain high amounts of ambient noises and possibly lower frequency human voices as left behind residue. 


\subsubsection*{Fast Fourier Transform}
We apply a Fast Fourier Transform(FFT) to the input data, consisting non-human-audible low-frequency audio clips, to compute features converting the signal from the time domain to the frequency domain. Like many real-time digital signal processing applications, the FFT must be computed on a shorter duration. As we will show in Section \ref{sec:expEval},  we set the FFT sample size to 256, resulting in a window size of 256/16000 = 0.016 seconds. 16 ms of signal data is short enough duration to produce a total of seven frequencies and their corresponding amplitudes as features for our models.

\subsubsection*{Prediction Module}
Finally, we employ standard machine learning techniques to predict mainly two characteristics of airflow: (1) The state of an air vent, as a binary classification problem predicting a discrete class label of the \emph{vent on or off} and (2) The rate of airflow, as a regression problem to predict the continuous values of airflow coming from the air vent. Note, however, that our regression model extends to execute the \emph{Minimum Persistence Scheme} (MPS), proposed in Section \ref{sec:MPS}. In doing so, MPS attempts to more accurately identify predictions that are highly likely to result from HVAC sound vibrations from other low-frequency ambient noises. 

We selected our parameters $n, p, \epsilon$, and $threshold$ for the minimum persistence and silence detection procedures by systematically testing combinations of parameters on a test data set, and selecting the parameters which yielded the best balance of accuracy improvement and model predictive ability.  Our final parameters for these procedures were $n=25, p=5, \epsilon=0.5, threshold=60$.

We note that the lowest accuracies for both naive and processed predictions correspond with the presence of human speech.  We hypothesize that this result corresponds with human speech activity within the \names range of $0-375$ Hz.  Other types of ambient noise, such as resonant noise from a laptop fan, music, and other types of relatively quiet ambient noise seem to have a lesser effect on the accuracy of our regression model.  Overall, the implementation of minimum persistence and silence detection enable our \names regression model to produce useful predictions even in the presence of audible and relatively frequent ambient noise.

==> introduction.old.tex <==
\section{Introduction}
\label{sec:intro}
%we depend on the infrastructure to support our health but this power can be determined by us, everyday occupant. convey importance of users to know how healthy indoor air is - e.g., water quality prashant's work. The solution to this is not obvious - e.g. SME cannot install sensors everywhere to accommodate to users.

Humans spend over 90\% of their lifetime in indoor spaces such as homes, office buildings, schools \cite{epa}. Healthy air hygiene is consequently essential for human health and comfort. One aspect of achieving healthy air is achieving proper ventilation. Being in poorly ventilated spaces can significantly harm one's health \cite{sundell2011ventilation}, for example, exacerbating respiratory problems such as asthma due to increased concentration of air pollutants \cite{epa}. Further, it can increase the spread of infectious diseases from accumulated viral loads in unregulated air. Improving indoor ventilation has gained renewed interest in recent years, especially since the coronavirus pandemic; COVID-19 has only proven how being physically present in a poorly ventilated space quickly increases one's risk of poor health outcomes. Accordingly, various health organizations such as the World Health Organization (WHO), Centers for Disease Control and Prevention (CDC) and The American Society of Heating, Refrigerating and Air-Conditioning Engineers (ASHRAE) recommended ways of improving indoor ventilation and measures to mitigate the spread of infections \cite{world2021roadmap,centers2021ventilation, ashraeOpen}. 

As we usher in a new era of informative health powered by internet-connected devices, more and more people have relied on sensing resources to help assess situations that may threaten their health—for example, using carbon dioxide sensors to measure CO\textsubscript{2} in the air or measuring ambient air temperature through smartphones \cite{aram2012environment,breda2019hot,devarakonda2013real, agarwal2011duty}. Despite many systems available to promote healthier air, the best solution may not always be evident to different stakeholders. To give an example, an institution will need to consider installing many carbon dioxide and temperature sensors that can support better indoor air quality for its everyday building occupant to keep abreast of their environment. Besides CO\textsubscript{2} and temperature, one piece of information critical to the user's understanding of healthier air is \emph{the rate of airflow}. As we witness advances in commodity devices to measure these parameters for user awareness, much remains to be learned in measuring airflow more conventionally.

The rate of airflow is measured using air meters and pressure sensors hard-wired in air ducts or near the air supply vents of standard HVAC systems. Research on improving HVAC systems is typically centered on energy efficiency, specifically achieving user comfort from utilizing efficient heating and cooling techniques \cite{chen2019gnu} and developing intelligent controls based on occupancy \cite{erickson2010occupancy, balaji2013sentinel}. But how much airflow is building occupants receiving in an indoor space? By knowing the airflow rate in a given area, users can be informed of how much fresh air is being replaced. Unfortunately, this information cannot yet be readily provided to everyday users.

While the dedicated setup of air meters and pressure sensors in supply air vents can effectively assist HVAC monitoring, it suffers from several drawbacks. First, buildings with older HVAC and ventilation systems may lack fine-grain monitoring capabilities in the air ducts. The addition of new hardware sensors in buildings is labor-intensive and expensive. Even so, these sensors may lose calibration over time, requiring commissioned building providers to provide regular maintenance. Finally, this setup is suitable for alerting facility managers to maintain an HVAC control system, which is not informative to everyday users about the airflow around them.

There is a need for a low-cost and non-intrusive sensing mechanism that measures the rate of airflow for the benefit of HVAC systems, facility managers, and building occupants themselves. With prior work leveraging mobile sensing techniques to estimate key indoor air quality parameters, our research similarly seeks to investigate the feasibility of measuring airflow. The larger goal of our work is to create an environmental health solution that can empower users with critical healthy air information to make better decisions of what buildings to enter while assisting the organization stakeholder to maintain standards. 

Given the properties of air as \emph{contactless} and \emph{ubiquitous}, acoustic sensing has the advantage to ``capture'' air. 
Thus, we hypothesize that \emph{the component of audio signals captured from a microphone sensor can be used to distinguish the rate of airflow in an indoor environment.} Fundamentally speaking, utilizing a mobile sensing device to measure air is not a new concept. Much work has proposed smart applications to support breath-by-breath analysis of airflow and detect respiratory airflow patterns primarily through a microphone sensor \cite{nam2015estimation, yadollahi2006robust}. 

The challenges we anticipate in designing this solution will be different, mainly since our application focuses on air circulating in the room in the vicinity of the user but not the air created by the user. As indoor environments are typically shared spaces, analyzing audio signals must prioritize user privacy. Second, the use case for human breathing requires users to place the microphone close to themselves as the source. In doing so, the audio of them breathing in and out will be the most prominent signal. In contrast, ours will require separating low amplitude moving air from the HVAC system and high amplitude ambient noise. It may also be impractical for users to align the microphone sensor closely with the HVAC system or air vent, especially if the sources are out of reach. Our solution to measure airflow should ideally operate wherever the users are located in the indoor space. Hence, we formulate the following research questions:
\begin{itemize}
    \item R1: Can we sense airflow using a microphone sensor in a privacy-preserving manner?
    \item R2: How robust is our solution in measuring airflow under different levels of indoor ambient noise?
    \item R3: What user factors mainly affect our solution's ability to measure airflow accurately?
\end{itemize}



%\missing{In order to measure the airflow from a vent, a variety of sensors can be used like accelerometer sensor, pressure sensor, microphone senor, etc. Among all of these, microphone sensor is the best choice as it is ubiquitous and does not need to be in contact with the vent to measure airflow. Existing work that uses microphone to sense breathing\cite{10.1145/3369835} strengthens our intuition of using the same sensor for monitoring airflow in indoor spaces. In this paper, we explore the feasibility of using microphone as an airflow sensor and study the factors that can affect its performance. We propose a system \names that monitors airflow in indoor spaces using off-the-she microphone. While the preliminary results are very promising, realizing \textit{FlowSense} is difficult due to the following challenges. First, Microphone captures all kinds of ambient noises from the environment. Thus, ambient noise interferes with the airflow signal affecting the system performance. Second, privacy is a major concern while using microphone sensor. There is always a trade-off between accuracy and privacy with many systems: reducing the amount of information available to ML models makes it more challenging to perform prediction tasks accurately. Third, the placement and orientation of the sensor w.r.t the vent might affect the sensing performance. Forth, as smartphone-sensing is bottle-necked by power concerns, we need to make sure that the system is power-efficient. Lastly, there are other factors that may affect the system performance like the movement and exposure of the microphone sensor, different types of vents, different microphone sensors/microphone-equipped devices.   }

%\begin{itemize}
   %\item R1: Can we sense airflow using a microphone sensor in a privacy-preserving manner?
    %\begin{itemize}
        %\item (a) Which part of the audio signal spectrum can give us accurate airflow rate estimation?%Which part of the audio signals and what frequencies are giving us high intensities of airflow?
        %\item (b) How do we ensure privacy while sensing airflow?%What is the most optimal ambient noise removal technique to employ?
        %\item (c) What characteristics of airflow can we accurately sense?
    %\end{itemize}
    %\item Can a microphone sensor also be used to sense the rate of airflow indoor in a privacy-preserving manner?
    %\item R2: How robust is our solution in measuring airflow under different levels of ambient noise?
    %\begin{itemize}
        %\item (a) Can we optimally eliminate ambient noise without compromising accuracy?%How do day-to-day noise in office environments affect the accuracy of our technique?
        %\item (b) What is the maximum boundary distance for the sensor placement without compromising accuracy?
    %\end{itemize}
    %\item R3: Which factors of consumers' smartphone characteristics mainly affect our technique's ability to measure airflow accurately?
%\end{itemize}

% In undertaking the investigation, we propose \name. This novel mobile sensing system employs a privacy-preserving pipeline of sampling audio signals collected from a microphone sensor. It utilizes a low-pass filter to analyze low-frequency signals of moving air. Further, our solution between sampling during silent periods and intelligently detects audio segments that contain persisting RMS noise of airflow. \names can successfully measure two airflow characteristics in rooms, specifically the status of an indoor air vent (as on or off) at 94\% accuracy and the rate of airflow at 92\% accuracy. Our model performance is influenced by the distance between the microphone and the air source. A sensor should ideally be within 2.5 meters away from the source to maintain accurate measures. Nonetheless, it proves robust in different environment and occupancy conditions.

In undertaking the investigation, we propose \name. This novel mobile sensing system employs a privacy-preserving pipeline of sampling audio signals collected from a microphone sensor. \names can successfully measure two airflow characteristics in rooms, specifically the status of an indoor air vent (as on or off) at 94\% accuracy and the rate of airflow at 92\% accuracy. Our model performance is influenced by the distance between the microphone and the air source. A sensor should ideally be within 2.5 meters away from the source to maintain accurate measures. Nonetheless, it proves robust in different environments and occupancy conditions.

We demonstrate the performance of \names through a feasibility study conducted in various indoor settings, accounting for room types, sources of ambient noises, and human conversations over a week. We also evaluate the effectiveness of our privacy-preserving pipeline among twelve participants rating the clarity of human audible speeches before and after our application processes them. Additionally, we carry out a case study from implementing \names as a smartphone application and testing the performance of sensing airflow in its real-world context.

To this end, we make the following contributions:
\begin{enumerate}[noitemsep,nolistsep]
    \item We design \names to determine the rate of airflow in an indoor space using a single-attribute microphone sensor. We comprehensively demonstrate \names to detect the status of air vents at 94\% accuracy and the rate of airflow at 92\% accuracy in a privacy-preserving manner.
    \item In achieving robustness to ambient noise, we propose the Minimum Persistent Scheme(MPS) as a dynamic thresholding technique to eliminate fluctuating predicted airflow rate beyond the lowest and constant predicted airflow rate, thus improving our accuracy by \missing{XX}\% when sensing airflow rate with the presence of ambient noise. The silent period-based sampling and the proposed MPS remove ambient noise's effect, improving system performance by \missing{XX}\%.
    \item We develop a \names as a mobile application for everyday users to measure the rate of airflow with commercial smartphones. Through an in-depth analysis, we characterize key user factors that will impact the performance of our solution, primarily the placement of sensor and smartphone hardware specifications.
\end{enumerate}

%We successfully overcome the above challenges by the following observations and designs. (i) The system samples only during silent periods and further filters the signal to ensure system privacy. (ii) We observe airflow is almost constant and continuous signal while ambient noise is variable and non-continuous. Based on this observation, we propose Minimum Persistent Scheme(MPS) that determines the lowest airflow rate predicted continuously over a period of time. In doing so, we naturally eliminate the *varying* value that may be unreasonably predicted due to ambient noise...minimum persisting value from a given range of predictions, thus making the system robust against ambient noise. The silent period-based sampling along with the proposed MPS removes the effect of ambient noise on the system performance. (iii) We identify major factors that can affect our system performance. We perform an in-depth analysis to study their effect on the system behaviour.




==> introduction.tex <==
\section{Introduction}
\label{sec:intro}
\update{Airflow measurement is a critical characteristic in ensuring healthy levels of air ventilation in any environment, particularly indoor spaces. With humans spending more than 90\% of their time indoors [X] and the recent COVID-19 outbreak exemplifying extreme health risks in poorly ventilated indoor spaces [X], measuring the airflow rate is fundamental in enabling proper ventilation to provide occupant comfort and safety [X].  To date, airflow measurement requires a limited selection tool such as vane, anemometer, and pressure sensors. These modalities are usually (a) expensive: they require dedicated installation near air supply vents, periodic maintenance, and re-calibrations, and (b) highly-specialized: they are intended for specialized uses by commissioned facilities management more than to benefit the community at large.}%

\update{Since ushering in the era of informative health powered by mobile sensing, much research efforts have successfully created rich, open sensing environments where people and municipalities can acquire real-time access to environmental data. For example, estimating CO\textsubscript{2} footprint using GPS mobility data \cite{XXX} or predicting ambient air temperature through smartphone batteries \cite{aram2012environment,breda2019hot,devarakonda2013real, agarwal2011duty}. In the same vein, we believe mobile sensing holds the potential to measure the rate of airflow in real-time. However, measuring airflow through a more common modality such as smartphones remains unattempted.}

\update{In its true nature, the properties of air are \emph{contactless} and \emph{ubiquitous}. While intangible, air carries sound, which is propagated as acoustic waves [X]. This basic principle guides our work to explore measuring the rate of airflow through acoustic-based mobile sensing techniques.} 

\update{Research in developing audio-based context recognition applications has evolved to provide broader user capabilities for daily activities [X], security [X], and more recently, health [X]. Regardless of the behavior of interest, such applications often are challenged by acoustic variability in audio signals. In these works, sensor data have been combined with data-driven AI and ML techniques to develop more robust audio models. For example, smart applications to support breath-by-breath analysis and detect respiratory airflow patterns primarily through a microphone sensor employ XXX, YYY...\cite{nam2015estimation, yadollahi2006robust}. Unlike prior work, the challenges we anticipate in measuring airflow through audio signals will be different, mainly since our application focuses on air circulating in the room in the vicinity of the user but not the air created by the user. As indoor environments are typically shared spaces, analyzing audio signals must prioritize user privacy. The use case for human breathing requires users to place the microphone close to themselves as the source. In doing so, the audio of them breathing in and out will be the most prominent signal. In contrast, ours will require separating low amplitude vibration sounds carried through air from the HVAC system and high amplitude ambient noise. It may also be impractical for users to align the microphone sensor closely with the HVAC system or air vent, especially if the sources are out of reach. Our solution to measure airflow should ideally operate wherever the users are located in the indoor space.}

\update{In undertaking the investigation, we propose \name. This novel mobile acoustic-based sensing system employs a privacy-preserving pipeline of sampling audio signals collected from a microphone sensor to measure the rate of airflow. We successfully overcome the aforementioned challenges by first sampling at a low rate of 16 kHz and applying a fast Fourier transform (FFT) algorithm to remove high-frequencies audio signals, a typical range for human speech. We further reduce our input data to only sample low-frequency sound vibrations from the HVAC during silent periods (i.e., when human speech is undetected), leaving us with a set of frequencies and their corresponding amplitudes as features. Our system utilizes the Gradient BoostingGradient ML algorithms to detect if an air vent is running (i.e., classification of on/off) and predicts airflow rate (i.e., regression). Due to low-frequency HVAC vibrations being in the same frequency range as many sources of indoor ambient noises, we introduce a dynamic thresholding technique, the \emph{Minimum Persistent Scheme (MPS)}, to more accurately distinguish predictions of HVAC sound vibrations from other low-frequency ambient noises. Unlike everyday ambient noises, the low-frequency HVAC vibration sounds lay constant over long periods. Thus, MPS attempts to determine the lowest airflow rate predicted continuously over a period of time as a threshold to eliminate fluctuating predictions. When go hand in hand, the silent period-based sampling and MPS can effectively separate predictions of HVAC airflow from other ambient noise effects.}

\update{We demonstrate the performance of \names achieving an overall accuracy of XX\% through a feasibility study conducted in various indoor settings, accounting for room types, sources of ambient noises, and human conversations over a week. We also evaluate the effectiveness of our privacy-preserving pipeline among twelve participants rating the clarity of human audible speeches before and after our application processes them. Additionally, we carry out a case study from implementing \names as a smartphone application and testing the performance of sensing airflow in its real-world context.}

To this end, we make the following contributions:
\begin{enumerate}[noitemsep,nolistsep]
    \item We design \names to determine the rate of airflow in an indoor space using a single-attribute microphone sensor. We comprehensively demonstrate \names to detect the status of air vents at 94\% accuracy and the rate of airflow at 92\% accuracy in a privacy-preserving manner.
    \item In achieving robustness to ambient noise, we propose the Minimum Persistent Scheme(MPS) as a dynamic thresholding technique to eliminate fluctuating predicted airflow rate beyond the lowest and constant predicted airflow rate, thus improving our accuracy by \missing{XX}\% when sensing airflow rate with the presence of ambient noise. The silent period-based sampling and the proposed MPS remove ambient noise's effect, improving system performance by \missing{XX}\%.
    \item We develop a \names as a mobile application for everyday users to measure the rate of airflow with commercial smartphones. Through an in-depth analysis, we characterize key user factors that will impact the performance of our solution, primarily the placement of sensor and smartphone hardware specifications.
\end{enumerate}

==> problem.tex <==
\section{Approach}
\label{sec:technique}
In this section, we justify the techniques we consider employing to overcome key design challenges in utilizing a microphone sensor for airflow prediction.\\

Broadly speaking, the most basic characteristic of continuously changing audio signals is the frequency range; \emph{low}, \emph{medium}, and \emph{high}. For example, the low-frequency range is between the limits of 10 Hz – 500 Hz \missing{[X]}, common as background noise attributed to the emission from manufactured sources such as computers, vehicles, or even HVAC systems. In actuality, sounds ranging from 20Hz are audible to humans. The mid-range boundary lies between 500Hz to \missing{XXX} Hz, capturing effective communicative sounds from a dog barking to a wide variety of male and female vocals \missing{[X]}. Finally, high-level frequencies range from  \missing{XXX}HZ to \missing{XXX}HZ. These sounds typically consist of musical overtones such as \missing{XXX}, \missing{XXX}, and \missing{XXX} \missing{[X]}. Clearly, the low-frequency audio spectrum is the most relevant to the essence of our research problem. However, separating signals from this frequency range alone is not a straightforward solution.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\columnwidth]{final_figures_only/Airflow_spectrums.png}
    \caption{Audio frequency spectrum under different rates of airflow and ambient noises.}
    %\vspace{-4mm}
    \label{fig:intuition_spectrum}
\end{figure}

\subsection{Preserving Privacy in Audio}
\subsubsection{Challenge}
Figure \ref{fig:intuition_spectrum} illustrates the audio frequency spectrum captured within an office space under multiple settings -- an unoccupied room with air ventilation turned on and off, with a variation of expected day-to-day office noises. We can visually inspect that the sound of moving air is approximately below the range of 500 Hz, and the signals remain somewhat consistent over time. 
%With the privacy of capturing human speech being a significant concern to our work, we can theoretically separate human speech by completely eliminating signals from mid-range frequency onwards. But how much of these frequencies should we eliminate when preparing audio clips for airflow measurement analysis?

\missing{To ensure privacy, we can use various. frequency domain or time domain techniques. In the time domain, it is possible to duty cycle the sampling and make the measured segments very short, so that it does not capture anything related to language syntax. 
In the frequency domain,} as the human speech frequency is overlapping with the airflow spectrum range, we can't separate the two spectrum simply by filtering. To ensure privacy, if we chose a filter such that it eliminates all human frequencies, then we will be left with very less features. So, there is an important question of how much of these frequencies should we eliminate when preparing audio clips for airflow measurement analysis? 


%\footnote{Audio recording is from a smartphone microphone, utilizing  Oxford SpectrumView 2.2 from Oxford Wave Research \cite{oxfordwave}, where the smartphone is held close (approximately 0.5 meters away) to a ceiling air vent with the screen facing upward.}; (a) an unoccupied room with no moving air from the air supply vent, (b) an unoccupied room with moving air from the air supply vent, (c) an occupied room with human audible speech and moving air, and (d) an occupied room with no human audible speech but human movements and machinery noises. 

To this end, we formulate our first research question: \textbf{\emph{R1: Can we sense airflow using a microphone sensor in a privacy-preserving manner?}} In answering this question, we seek to determine (a) which part of the audio signal spectrum can give us accurate airflow rate estimation? (b) How can we ensure privacy while sensing airflow? With a privacy-preserved audio spectrum left to analyze, (c) what characteristics of airflow can we accurately sense?

\subsubsection{Technique: Sampling Rate and Low-pass Filter}
%For most audio applications, 44.1 kHz is the optimal sample rate because it allows the reproduction of all sounds below the 22.05 kHz threshold, as stated by the Nyquist theorem \missing{[X]}. Any noise above 22.05 kHz is considered inaudible \missing{[X]}. For this reason, we will begin our experiment with the lowest sampling rate of 8000Hz on the microphone to obtain only low-frequency sounds. 

To isolate a low-frequency band, we can employ a low-pass filter, but must consider the accuracy-privacy trade-off from reducing data dimensionality. From the accuracy perspective, an increased cut-off frequency gives us more feature information to produce better predictions. However, additional frequencies could conceivably interfere with the airflow signal, thus compromising accuracy. Conversely, reducing feature information also result in more coarse-grained features and impact prediction performance. From the privacy perspective, we want the cut-off frequency to be as low as possible to avoid capturing audible noise(especially speech) in the environment. Hence, determining the optimal cut-off frequency for the low-pass filter is essential. In Section \missing{XXX}, we empirically demonstrate how the sound of airflow in audio signals is broadly between 0-500 Hz, thus, limiting our cut-off frequency within this range. Ideally, the cut-off frequency for our low-pass filter should guarantee privacy by not detecting any human audible speech. 



In Section \missing{XXX}, we conduct a feasibility study to determine the optimal sampling rate and cut-off frequency for the low-pass filter to ultimately preserve privacy in audio-sensing.

\subsection{Eliminating Ambient Noise}
\label{sec:challenge_ambient}
\subsubsection{Challenge}
In actuality, low-frequency noise is composed of different day-to-day sources within the environment \missing{[X]}. One significant challenge we foresee in relying on low-frequency audio signals is distinguishing noise produced by the HVAC system from other manufactured sources, including office machinery (e.g., photocopier, printer, or moving vehicles), moving vehicles, talking, and other everyday ambient noises (as shown in Figure \ref{fig:intuition_spectrum}). Accordingly, our second question aims to answer, \textbf{\emph{R2: How robust is our solution in measuring airflow under different levels of ambient noise?}} 

\missing{Ambient noise is a major challenge for our system as it leads to incorrect predictions. This ambient noise may include speech, machine noises, and other day-to-day noises in an indoor environment. A possible way to remove the speech frequencies is to look at its harmonics in the higher frequency spectrum. But this would require looking at high frequency spectrum that may result in privacy concerns. Another way to address this problem is to apply decibel thresholding on a segment of spectrum or the entire spectrum to remove noise above a certain threshold. As this might not remove very low ambient noises, so we  propose a techniques that further removes the effect of ambient noise by leveraging the nature of airflow in indoor environment. To this end, we propose two techniques to improve the system accuracy in presence of ambient noise.}

\subsubsection{Technique \#1: Silent Periods}
\label{sec:silentperiods}
It is theoretically feasible for our solution to mainly ``watch out'' for periods where minimal ambient noise is present to measure the rate of airflow. 

Figure \ref{fig:noisegap_spectrum} illustrates the audio signals of three indoor settings with different sources of ambient noise we expect to encounter: (a) a mid-sized room with several humans conversing and laptop/projector running (e.g., a meeting), (b) a crowded large-sized room with a principal speaker (e.g., conference room or lecture hall), and (c) a crowded large-sized room with multiple ongoing conversations (e.g., cafeteria). Through (a) and (b), we observe structures of pauses that commonly exist in audio signals. However, these ``silent gaps'' are less apparent in crowded areas. A preliminary analysis of these audio signals found distinct gaps from as much as ten seconds to as little as ten milliseconds (ms). However brief they may be, these silent gaps can be the desired sampling period. 

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\columnwidth,height=2cm]{figures/spectrum_noiseGap.jpg}
    \caption{\missing{Audio frequency spectrum involving human speech shows presence of silent gaps.}}
    %\vspace{-4mm}
    \label{fig:noisegap_spectrum}
\end{figure}

By first determining the maximum root mean squared (RMS) noise of air coming from the vent, we can set the RMS noise as a threshold to detect silent periods and collect audio samples for airflow. 
%Since human speech can fall in the low-frequency range, this technique can be a workaround to preserve privacy.
While we expect this method to produce the most accurate measure of airflow, prediction capability may fail drastically in loud indoor environments. 

\subsubsection{Technique \#2: Minimum Persistent Scheme}
\label{sec:mpsdescription}
Indeed, knowing the optimal rate of airflow becomes increasingly important as an indoor space gets filled with occupants, thus, exposed to more ambient noises. It is equally essential that further reducing our sample does not affect the feasibility and efficacy of our solution. For this reason, we investigate a second technique of finding the minimum persisting airflow value amongst \textit{n} consecutive predictions.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\columnwidth]{final_figures_only/intuition_ambientNoise.png}
    \caption{\missing{The amplitude of the sound waves of moving air from vents and office machines.}}
    %\vspace{-4mm}
    \label{fig:intuition_ambientnoise}
\end{figure}

Inspecting the low-frequency spectrum from a different perspective in Figure \ref{fig:intuition_ambientnoise}, we observe a notable aspect to differentiate air supplied from the office vent and other surrounding noises. 
The airflow signal involves minimal fluctuations in pressure that the waves remain relatively constant over a significant period while ambient noise varies a lot. Thus, the airflow signal appears continuous, while ambient noise is discrete. Assuming our audio samples contain discrete values of ambient noises, our model is likely to over-predict the rate of airflow. 

\subsection{Practical Considerations}
The broader goal of our work aims to provide the need for everyday use among everyday users. Using the microphone as a sensing modality, we expect our solution to work without requiring technical expertise and dedicated installation. Our third research question aims to understand, \emph{\textbf{R3: What user factors mainly affect our solution’s ability to measure airflow accurately?}}

\subsubsection{Smartphone Compatibility \& Capability}
%Our final challenge aims to address, \textbf{\emph{R4: Which factors of consumers' smartphone characteristics mainly affect our technique's ability to measure airflow accurately?}}
With smartphones regarded as commodities and these devices having more than one microphone sensor, our investigation continues with leveraging microphones in-built smartphones for any user to conveniently measure airflow when in an indoor location. However, today's wide variety of smartphone models have different sensor capabilities, primarily based on the manufacturer's design and device price range. Additionally, with users handling their smartphones just about any way they wish to (i.e., walking, standing, in-pocket, different positions, and orientations), we need to consider how these variations mainly affect the performance of our solution.
 
\subsubsection{Sensor Installation Placement}
In its current state-of-the-art form, the airflow sensor requires much care and attention in mounting and placement on HVAC systems to ensure the device achieves its appropriate purposes (e.g., measure volume of air, the mass of air, and wind direction). The ideal arrangement is for the sensor to be at the center of the duct. However, it demands meticulous expert consideration, such as system vibrations, debris, and turbulent locations \missing{[X]}. Our solution cannot afford the technical calibrations required by typical airflow sensors to cater to everyday users. At the very least, the microphone sensor can be placed anywhere a user likes.
\begin{wrapfigure}{r}{.5\linewidth}
\centering
    \includegraphics[width=\linewidth]{final_figures_only/intuition_distanceamplitude.png}
    \caption{\missing{The amplitude of the sound wave of moving air decreases with distance from its vent source.}}
    %\vspace{-4mm}
    \label{fig:intuition_amplitude}
\end{wrapfigure}

A practical question we seek to address in this work is to determine how far away the microphone sensor should be placed from the air vent. Fundamentally, as sound waves propagate away from the source, sound intensity decreases \missing{[X]}. As shown in Figure \ref{fig:intuition_amplitude}, since sound intensity is proportional to the square of the amplitude of waves, we can expect the amplitude of sound waves to decrease with increasing distance from the air vent source \missing{[X]}. However, the maximum spatial boundary our sensing technique is limited to before accuracy is compromised remains unknown.



In addressing these practical considerations, we comprehensively examine the performance of our solution under various indoor and smartphone setups. We explain them in Sections \missing{XXX} and \missing{XXX}, respectively.

==> smartphone.tex <==
\clearpage
\section{Smartphone Implementation}
\label{sec:casestudy}
We extend our efforts to realizing \names as a smartphone app.Figure \ref{fig:casestudymain} depicts our implementation and the optimal smartphone device placement and orientation, balancing system performance and ease of use. In what follows, we explain our experiment results in detail.
\begin{figure}[h!]
    \centering
    \includegraphics[width=.7\linewidth]{final_figures_only/casestudysetup.png}
    \vspace{-1em}
    \caption{\names smartphone implementation, showcasing optimal application use.}
    \label{fig:casestudymain}
\end{figure} 

\subsubsection*{Study Procedure}
Our study involves four Android smartphone devices - one device for training (i.e., Tr) our \names mobile model and three devices for test (i.e., Tt). These devices are \textbf{Tr-1}(LG Stylo 4, Snapdragon 450 @ 1.8 GHz, 2GB RAM, Android version 8.1), \textbf{Tt-1} (Samsung Galaxy S8, Snapdragon 835 @ 2.35 GHz, 4GB RAM, Android version 9.0), \textbf{Tt-2} (Google Pixel XL, Snapdragon 821 @ 2.15 GHz, 4GB RAM, Android version 10), \textbf{Tt-3} (OnePlus One, Snapdragon 801 @ 2.5 GHz, 3GB RAM, Android version 6.0). As indicated in Figure \ref{fig:casestudymain}, we paired \textbf{Tr-1} with an Arduino Nano 33 BLE Sense to relay ground truth airflow readings from the Rev. P wind sensor (same as our device setup in the feasibility setup). Unlike our feasibility study, which was conducted in a controlled environment, we describe our app's performance under multiple indoor environments with varying ambient noise in Section \ref{sec:indoorenv}.

\subsubsection*{Dataset} Our training dataset consists an equal proportion of data that measured at varying distances, orientation and indoor environment. These are key variables in the later parts of our experiments. \missing{For each model, 20\% of these training datasets were set aside as test data for each model, leaving 31,200 training points for the regression model, and 64,000 training points for the classification model.}
%All datapoints from Tr1 for training, 20% test for Tr-1 random sampling). XX minutes == XXk datapoints.
%Dataset for Tt1-4: estimate of average for each phone. 20 minutes, no more than 20,000 data points.
%classification, recorded for no airflow (estimate of how long this is-30 minutes addition of no airflow).

\subsection{Smartphone App Performance}
\label{sec:modelarch}

%Figure \ref{fig:mobilesystem} illustrates our replication of the feasibility study into a smartphone application. As we will later explain in Section \ref{sec:devicepos}, our app must extend a context awareness module, which senses device movement, orientation, and phone exposure. This module infers phone movement and orientation using a standard accelerometer API. In contrast, we measure phone exposure using proximity and light sensor APIs, accessible through the SensorManager framework. We implement our prediction models using \emph{scikit-learn} Python framework, and \emph{Noise} wrapper for \emph{kissfft} FFT computation library \cite{noise,kissfft}. Finally, we utilize the \emph{JPMML} project to convert our Python-trained model into a Java-compatible object, allowing the computation of predictions directly on the smartphone \cite{jpmml}.

Table \ref{tab:smartphone_model} summarizes our model performance through two validations, 5-fold CV and test. Overall, we observe above 90\% accuracy in predicting vent status \missing{(difference is non-significant). Similarly, we maintained above 0.9 regression score in predicting the rate of airflow. This difference, however, is significant at XXX.}\todo{after looking at the scikit-learn documentation, I'm not sure that the "train" data is cross validated at all.  I can share the code to show where these numbers come from}

\begin{table} [!h]
\scalebox{.8}{
\centering
  \begin{tabular}{|l|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\makecell{\textbf{Prediction}}} &
      \multicolumn{4}{c|}{\textbf{Classification}} &
      \multicolumn{2}{c|}{\textbf{Regression}} \\
      & Acc & Prec. & Rec. & F1 & MSE & Reg. \\ \hline
      Vent on/off: Tr-1 & 0.961 & 0.960 & 0.961 & 0.961 & \cellcolor{black!60} &  \cellcolor{black!60}\\\hline
      Vent on/off: Test & 0.911 & 0.916 & 0.907 & 0.907 &
      \cellcolor{black!60} & \cellcolor{black!60} \\\Xhline{2\arrayrulewidth}
      Vent on/off: Avg Test 4 & 0.911 & 0.916 & 0.907 & 0.907 &
      \cellcolor{black!60} & \cellcolor{black!60} \\\Xhline{2\arrayrulewidth}
      Rate of Airflow: 5-fold CV &\cellcolor{black!60} & \cellcolor{black!60} & \cellcolor{black!60} & \cellcolor{black!60} & 0.488 & 0.991 \\\hline
      Rate of Airflow: Test &\cellcolor{black!60} & \cellcolor{black!60} & \cellcolor{black!60} & \cellcolor{black!60} & 3.938 & 0.927 \\\Xhline{2\arrayrulewidth}
  \end{tabular}}
  \caption{Performance comparing train and test of our classification and regression models.}
  \label{tab:smartphone_model}
\end{table}

\subsection{Device Distance and Orientation }
\label{sec:devicepos}

It is most practical for users to hold their smartphones in any preferred way when utilizing \names app. This first experiment investigates how different device placement and orientation affect our model performance. It attempts to determine the most comfortable way to place the device to receive optimal results.

\begin{table} [!h]
\scalebox{.8}{
\centering
  \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\makecell{\textbf{Orientation/Distance}}} &
      \multicolumn{5}{c|}{\makecell{\textbf{Vent Status}\\(Classification, Accuracy)}} &
      \multicolumn{5}{c|}{\makecell{\textbf{Rate of Airflow}\\(Regression, MSE)}} \\
      & 0.5m & 1.0m & 1.5m & 2.25m & 3.0m & 0.5m & 1.0m & 1.5m & 2.25m & 3.0m \\\Xhline{2\arrayrulewidth}
      0° (microphone upwards facing vent) & 0.983 & 0.957 & 0.945 & 0.928 & 0.821 & 0.63 & 0.72 & 0.73 & \cellcolor{green!25}0.97& 1.12
      \\ \hline
      90° (microphone perpendicular to the vent) & 0.960 & 0.944 & 0.889 & 0.953 & 0.942 & 0.62 & 0.84 & 0.73 & 0.64 & 0.74\\ \hline
      180° (microphone downwards facing away from the vent) & 0.962 & 0.955 & 0.822 & 0.842 & 0.524 & 0.55 & \cellcolor{green!25}0.71 & 0.46 & 0.57 & 0.95 \\ \hline
  \end{tabular}}
  \caption{Performance of predicting vent status and rate of airflow at varying distances.}
  \label{tab:distorient}
\end{table}

%OLD VALUES WITHOUT MPS
% \begin{table} [!h]
% \scalebox{.8}{
% \centering
%   \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%     \multirow{2}{*}{\makecell{\textbf{Orientation/Distance}}} &
%       \multicolumn{5}{c|}{\makecell{\textbf{Vent Status}\\(Classification, Accuracy)}} &
%       \multicolumn{5}{c|}{\makecell{\textbf{Rate of Airflow}\\(Regression, MSE)}} \\
%       & 0.5m & 1.0m & 1.5m & 2.25m & 3.0m & 0.5m & 1.0m & 1.5m & 2.25m & 3.0m \\\Xhline{2\arrayrulewidth}
%       0° (microphone upwards facing vent) & 0.983 & 0.957 & 0.945 & 0.928 & 0.821 & 0.96 & 2.02 & 2.58 & \cellcolor{green!25}1.27 & 3.40 \\ \hline
%       90° (microphone perpendicular to the vent) & 0.960 & 0.944 & 0.889 & 0.953 & 0.942 & 1.25 & 1.46 & 1.48 & 2.69 & 2.39 \\ \hline
%       180° (microphone downwards facing away from the vent) & 0.962 & 0.955 & 0.822 & 0.842 & 0.524 & 1.10 & \cellcolor{green!25}0.79 & 1.15 & 2.22 & 2.02 \\ \hline
%   \end{tabular}}
%   \caption{Performance of predicting vent status and rate of airflow at varying distances.}
%   \label{tab:distorient}
% \end{table}

We modulate \emph{distance} and \emph{orientation}, as two primary parameters affecting our models' performances. Distance is two points between the smartphone's microphone to the HVAC vent, with the nearest being 0.5 meters away. Orientation is relative to the frame of reference, in this case, the HVAC vent. 0° is the smartphone microphone facing towards the vent, 90° is the smartphone microphone facing along an axis perpendicular to the vent (e.g. given a ceiling-mount vent, the primary microphone faces one of the room's walls), 180° is the smartphone microphone facing away from the vent.

%Distance first
\subsubsection*{Increasing Error with Distance} 
Table \ref{tab:distorient} summarizes our model performances in predicting vent status and airflow rate at different distances and orientations. Our classification model is 90\% accurate in informing users if the vent is running as long as the smartphone is within 3.0m (p<0.05) from the air vent—the increasing distance results in incremental drops. Additionally, results from our regression model yields slight inconsistencies between 0.63-0.97 MSE with increasing distance. Our regression model performance is significantly affected at 3.0m apart \missing{(p<XXX)}. In a typical situation where a user stands up and holds the microphone smartphone roughly 2.25m away and facing the vent (0° device orientation), \names yields 0.97 MSE, in which the difference is non-significant compared to being 0.5m apart.

%Orientation second
\subsubsection*{Unobstructed Microphone Oriented Towards Vent} 
Device orientation is also a factor that will affect our model performance. Specifically for our classification model, we observe significant drops below 80\% accuracy \missing{(p<XXX)} when the microphone lies obstructed from audio signals. This condition strongly implies that \names cannot operate as intended should the phone be unexposed (e.g., in the user's pocket), thus, informs our decision to implement context-awareness capabilities as a compulsory module of our app -- see Figure \ref{fig:mobilesystem}.

In contrast to our classification model, our regression model is unaffected by device orientations because \missing{...provide reason as to why.} 
%We notice a drop in accuracy around 2.25m, particularly when the smartphone is positioned at 180 degrees, and a general drop in accuracy across all orientations for distance 3 meters.

\todo{which one is this corresponding to?}Using 12 datasets for each distance, each with 1000 data points, we find that the difference in classification accuracy between 50cm and 1m is statistically significant.  The difference in accuracy between 1m and 1.5m is not statistically significant, and although the difference between 1m and 2.25m is statistically significant, we find that the model's performance on specifically 2.25m data at 90 degrees orientation is very similar to the model's performance at 1m, and does not entail a statistically significant difference.  We consider 2.25m at 90 degrees to be an important metric as it is a standard distance \& orientation for a smartphone placed on a table. 

%In order to analyze performance in a variety of these situations, we collect test data with ground truth airflow readings for each (distance, orientation) permutation.  For the regression model, we compare \names predictions with the recorded ground truth values, using mean squared error and regression score as metrics.  For classification, we label our test data according to the airflow situation it was recorded in, and check \names classification results using accuracy, precision, and recall as metrics.\\




%\ncz{how is phone placed on a table with its screen facing upwards giving higher MSE than microphone pressed down on the table?} \missing{I think the conclusion that we came to for this question was that accuracy was better at 180 degrees (2.25m) because the phone and the groundtruth sensor are basically experiencing near-zero airflow values at this large distance away from the vent, and therefore the collected data is consistent and easy to infer airflow values for}.

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.7\columnwidth]{final_figures_only/bar_plot_with_error_bars.png}
%    \vspace{-1em}
%    \caption{Performance of Regression Model at different device distances and orientations}
%    \label{fig:distorient}
%\end{figure}

Based on these empirical results, we conclude that the optimal range of distances from the HVAC vent for both \names classification and regression models lies between 0.5m and 2.25m -- this range is a wide enough range to encompass many real-world situations that a smartphone may be placed in.  

%In these experiment runs, all phones are assumed stationary.  As discussed in section \ref{sec:modelarch}, we recommend coupling the application with context-aware capabilities sensing for user activity, phone exposure, and device orientations in a full-fledged implementation.

%Each FFT calculation takes as input a frame containing 256 samples. An FFT of size 256, given a 16 kHz sampling rate, results in a frequency resolution of 62.50 Hz, as required by our trained model.

%Training data was collated from the ground truth dataset that we recorded using the ground truth setup on a single training vent, with P1, an Arduino, and the Rev. P wind sensor.  For each model, an equal proportion of each category of data was included in the training set -- categories included distance and orientation, as described in section \ref{sec:pos}, and data that was labeled according to whether groundtruth airflow was present or not.  20\% of these training datasets were set aside as test data for each model, leaving 31,200 training points for the regression model, and 64,000 training points for the classification model.







%In Figure \ref{fig:mobilesystem}, we visualize the deployed architecture of the \names regression and classification models on a smartphone.  We include a \textit{context awareness module}, which senses for user activity, phone exposure, and device orientation. Phone movement and orientation is inferred using a standard accelerometer API, while phone exposure is measured using proximity and light sensor APIs -- on Android, all such sensors are accessible through the \emph{SensorManager} framework. \names will not begin the process to sense a sample unless the necessary conditions of the device being stationary, exposed, and adequately oriented are met.

\subsection{Smartphone Model Variation}
We expect different smartphone devices to affect our model performance since smartphones are likely to integrate different microphone specifications. For example, smartphones with microphones that are intended for voice-only recordings tend to have lower cutoff frequency, thus producing different \textit{frequency response}, which may intuitively affect our model accuracy. Our experiment considers several smartphone models (i.e., \textbf{Tt-1}, \textbf{Tt-2}, \textbf{Tt-3} and \textbf{Tt-4}), explicitly for test (of our trained model using \textbf{Tr-1}). 
%Combined with the training device P1, the four devices chosen represent a holistic cross-section of the Android installed base, with a wide variety of capabilities, software versions, and hardware limitations.  The following devices were used to evaluate \names on devices which the model had not been trained on:

%\scalebox{0.7}{
\begin{table}[h!]
\begin{tabular}{|l|c|c|c|c|c|}\hline
 & \textbf{Tr-1} & \textbf{Tt-1} & \textbf{Tt-2} & \textbf{Tt-3} & \textbf{Tt-4} \\
  & LG Stylo 4 & Samsung Galaxy S8 & Google Pixel XL & OnePlus One & LG Stylo 3 \\ \hline
\textbf{Regression MSE} & 0.439 & 0.486 & 0.656 & 0.680 & 27.64\\ \hline
\textbf{Classification Acc.} & 0.941 & 0.194 & 0.724 & 0.884 & 0.345\\ \hline
\textbf{Runtime} & 3.1 ms & 2.9 ms & 2.9 ms & 3.4 ms & 3.3 ms\\ \hline
\end{tabular}
\caption{Accuracy (in MSE) and processing time (in milliseconds) of \names on four different smartphone devices. }
\label{tab:smartphone_model}
\end{table}
    

Fig. \ref{tab:smartphone_model} tabulates the overall accuracy (measured in MSE) and \names computation time on the four different smartphones.  On most of the smartphones tested, \names is able to achieve a low mean-squared error for the regression model.  

During our testing, we noticed minute variations amongst the \textit{frequency responses} of some smartphones.  Some different smartphone models, when recording microphone data in an identical environment, reported slightly different noise amplitudes for specific frequencies -- intuitively, if the smartphone's frequency response differs within the \names model range of 0-375 Hz, we anticipate the accuracy of our models to decrease.  For classification, we hypothesize that this phenomenon causes the \names classification model to perform poorly on P2.  For deployment of our system, we recommend that the differences in frequency response amongst devices be studied and understood.

\subsection{Energy Consumption}
\label{sec:energycons}

To examine the impact of \names on battery life, we conduct a study into the energy consumption of the entire \names stack, including the mobile application itself and OS-level APIs for sensing, including microphone audio stream and orientation/movement sensors.  We compare this energy consumption against a baseline value consumed by the usual Android background processes and wireless radio.  Using the Android project's \textit{Battery Historian} tool to measure energy usage, in our testing on Tr-1, the entire \names stack, under continuous sensing, consumed 6.08 mA/h of energy.  In the same conditions, Android System background processes and the cellular wireless radio used 6.6 mA/h of energy.  

Using duty cycling, we can significantly mitigate the energy effects of \name.  By sensing for one minute at a time, separated by set intervals, we decrease the energy usage of \names -- sensing once every 10 minutes yields energy usage of 0.61 mA/h.  Compared against the baseline, this duty cycling increases background energy consumption on Tr-1 by less than 10\%.  Considered jointly with the battery capacities of contemporary smartphones, which often have capacities in excess of 2000 mAh, we conclude that the background energy impact of \names would be easily manageable.

\subsection{Common Indoor Environments}
\label{sec:indoorenv}
\subsubsection*{Room Conditions}
We consider the real world performance of \names in a variety of states which the system would likely be deployed.  We consider two main distances from the main HVAC vent in the room, at $0.5m$ and $2.25m$, meant to approximate positions where the smartphone is being held towards the vent, and where the smartphone is lying horizontally on a table in the room, respectively.  For each of these distances, we also consider whether or not the room is \textit{occupied}, which we define, for this experiment, as having either no individuals or $\ge 2$ individuals in the room.\\
Fig. \ref{fig:realworldphone} tabulates the accuracy, precision, and recall of the \names classification model for these different conditions, as well as the corresponding mean squared error and regression score for the \names regression model.  Results are grouped into sections based on the smartphone that was used for each dataset.\\
Fig. \ref{fig:plotrealworld} plots the actual regression results for predicting the rate of airflow in a mixed set of situations.  In Region 1, we see a case where \names slightly under predicts airflow -- this may occur when ground truth airflow is very high, as high rates of airflow are generally unlikely in the average indoor environment.  In Region 2, we see a case where \names slightly over predicts airflow -- this can occur due to the presence of ambient noise, as discussed in section \ref{sec:expamb}.  In Region 3, we show that in the average case, \names regression model achieves a high degree of accuracy in airflow rate prediction.

\begin{figure}[h!]
    \centering
    \scalebox{.8}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|}\hline
    \toprule
    \textbf{Experiment Setup} & \textbf{Classification Acc.}  &  \textbf{Regression MSE}\\
    \toprule
    \textbf{Unoccupied} with P1 at \textbf{0.5m} away from vent & 0.863 & 2.68 -> 0.724 \\
    \textbf{Occupied} with P1 at \textbf{0.5m} away from vent  & 0.86 & 3.12 -> 0.731 \\
    \textbf{Unoccupied} with P1 on table at \textbf{2.25m} away from vent & 0.946 & 2.59 -> 0.636 \\
    \textbf{Occupied} with P1 on table at \textbf{2.25m} away from vent & 0.95 & 6.53 -> 0.926 \\
    \textbf{Occupied} with P1 \textbf{in hand}, roughly \textbf{2m} away from vent & 0.78 & 6.61 -> 4.54 \\\hline
    \textbf{Unoccupied} with P2 at \textbf{2.25m} away from vent & 0.19 & 0.49 \\
    \textbf{Unoccupied} with P3 at \textbf{2.25m} away from vent & 0.74 & 0.66 \\
    \textbf{Unoccupied} with P4 at \textbf{2.25m} away from vent & 0.88 & 0.68 \\\hline
    \end{tabular}} 
    \caption{Real world performance of classification and regression models}
    \label{fig:realworldphone}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\columnwidth]{regressionPrediction.png}
    \caption{\names regression model performance on a diverse set of ground truth airflow values.  We split the figure into three regions, showing cases that may arise when \names is deployed.  In the average case, the regression model is able to predict values for airflow quite well.}
    \label{fig:plotrealworld}
\end{figure}

\iffalse
\subsubsection*{Bucketizing}

\missing{Discuss Bucketizing, introduce and discuss plot of accuracies}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\columnwidth]{bucketexample1.png}
    \caption{Performance of Regression Model with Bucketizing for different groundtruth rates of airflow}
    \label{fig:distorient}
\end{figure}

Discussion of bucketizing parameters and accuracy
\fi



% \subsubsection{Smartphone Variations}
% Add results for both Generalized and Personalized

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\columnwidth]{figures/Screen Shot 2021-09-07 at 17.48.20.png}
%     \caption{Model generalization for different smartphones}
%     \label{fig:my_label}
% \end{figure}



\subsubsection{Effect of Ambient Noise}\label{sec:expamb}

Recall Section \ref{sec:challenge_ambient}. We listed some examples of scenarios in which our system will be utilized and respond, analyzing some cases of ambient noise that we can expect \names to be faced with.  We broadly categorize indoor situations users are likely to be in; (1) a mid-sized room with multiple individuals conversing (e.g., a meeting), (2) a mid-sized room with two individuals engaged in a conversation, (3) an office environment with typical noises of office machines (example - laptop/computer fan), (4) music played through a laptop speaker in close proximity to the smartphone, (5) speech played through a laptop speaker (example of video or teleconferencing), and (6) street or city noises approximating the effect of an open window or loud environmental noise.

In real ambient noise cases, we created the corresponding environment and recorded test data with ground truth airflow readings, concurrently recording average dB sound levels in the smartphone's area.  For conversation noise cases, we recorded this test data in the context of a real meeting, with the corresponding number of individuals.  For the office background noise case, we placed a PC laptop with a fan running at 100\% speed, 50cm away from the smartphone.  In each real ambient case, we recorded at least 20 minutes of data.

To record synthetic ambient noise, we placed a fanless laptop computer 1m away from the smartphone and ground truth airflow setup.  Using a fixed volume setting, we played a sound file corresponding to each ambient noise case through the laptop's speaker, concurrently recording the average dB sound levels in the smartphone's area.  In each synthetic ambient case, we recorded at least 20 minutes of data.  \missing{cite sound files / youtube videos used for this} 

For each of these synthetic and real ambient noise cases, we evaluate the performance of the \names regression model using mean squared error as a metric for accuracy.  

In Fig. \ref{fig:smartphone_speechtype}, we tabulate our accuracy results for each of these ambient noise cases.  As predicted in section \ref{sec:challenge_ambient}, the presence of ambient noise causes the naive predictions of the \names regression model to over predict airflow in the environment, resulting in relatively high MSE, and corresponding with poor accuracy.

Leveraging the information detailed in \ref{sec:mpsdescription}, we implement a minimum persistence algorithm that takes as input some sequence of continuous samples, of size $n$.  Since we are only interested in the points where ambient noise is not present, we report the minimum non-outlier prediction obtained from the $n$ samples in the sequence.  We introduce two parameters; persistence parameter $p$ and threshold parameter $\epsilon$ which attempt to capture a common minimum value from our model.  Given the sequence of $n$ numbers, we sort the predictions in ascending order, and subsequently attempt to find a "window" of values with size $p$, such that $p$ consecutive values are all within $\pm \epsilon$ of the window's average value.  The algorithm then reports this value as the prediction for all $n$ samples, or, if such a window cannot be found, simply terminates and waits to receive a new batch of $n$ samples.

In Fig. \ref{fig:casesambbar}, we show that implementing a minimum persistence and silence detection procedure as described in sections \ref{sec:silentperiods} \& \ref{sec:mpsdescription} achieves a large reduction in MSE, corresponding to an increase in accuracy of between 78-98\%.  We selected our parameters $n, p, \epsilon$, and $threshold$ for the minimum persistence and silence detection procedures by systematically testing combinations of parameters on a test data set, and selecting the parameters which yielded the best balance of accuracy improvement and model predictive ability.  Our final parameters for these procedures were $n=25, p=5, \epsilon=0.5, threshold=60$.

We note that the lowest accuracies for both naive and processed predictions correspond with the presence of human speech.  We hypothesize that this result corresponds with human speech activity within the \names range of $0-375$ Hz.  Other types of ambient noise, such as resonant noise from a laptop fan, music, and other types of relatively quiet ambient noise seem to have a lesser effect on the accuracy of our regression model.  Overall, the implementation of minimum persistence and silence detection enable our \names regression model to produce useful predictions even in the presence of audible and relatively frequent ambient noise.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\columnwidth]{figures/Screen Shot 2021-09-07 at 17.48.26.png}
%     \caption{Effect of Ambient Noise on performance of classification and regression models}
%     \label{fig:my_label}
% \end{figure}

\begin{center}
\textit{Cases of Ambient Noise}\\
\end{center}
\textbf{Actual ambient noise}
\begin{itemize}
    \item Case 1: Three person discussion -- 56 dB average noise level
    \item Case 2: Two people -- conversation -- 58 dB average noise level
    \item Case 3: Office machine noise -- laptop fan -- 46 dB average noise level
\end{itemize}
\textbf{Simulated ambient noise}
\begin{itemize}
    \item Case 4: Music background through speakers -- 55 dB average noise level
    \item Case 5: Conversation through speakers -- 53 dB average noise level
    \item Case 6: Street/white noise through speakers -- 50 dB average noise level
\end{itemize}

\begin{figure}[ht!]
\begin{tabular}{|l|l|c|c|}\hline
\textbf{Case} & \textbf{Environment} & \textbf{Speech/Noise-level} & \textbf{MSE}\\ \hline
1 & Three person conversation in a meeting room \textbf{56 dB avg.} & Audible & 0.746 \\
2 & Conversation between two people in a mid-sized room \textbf{58 dB avg.} & Audible & 0.547 \\
3 & Office background noise (laptop computer fan) \textbf{46 dB avg.} & White noise & 0.768 \\ \hline
4 & Music background noise (through laptop speaker) \textbf{55 dB avg.} & Audible & 0.535 \\ 
5 & Speech (through laptop speaker) \textbf{53 dB avg.} & Audible & 0.916 \\
6 & Street/City noise (through laptop speaker) \textbf{50 dB avg.} & White noise & 0.442 \\ \hline 
\end{tabular}%} 
\caption{Accuracy, measured in mean squared error, of \names regression with various levels of ambient noise. }
\label{fig:smartphone_speechtype}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\columnwidth]{final_figures_only/bar_plot_with_error_bars_noise.png}
    \vspace{-1em}
    \caption{Performance of Regression Model with different cases of simulated and real ambient noise}
    \label{fig:casesambbar}
\end{figure}

\section{Discussions}
\textit{Applications and Scope}. The proposed system is the first step towards creating healthy indoor environment and giving the power to the occupants to know the environment around them. We envision that this work can be further extended to find the Air changes per hour(ACH) in indoor environment by utilizing additional information about the room dimensions and vent specifications. This will enable users to know whether the indoor environment around them is safe or not. If there is an indoor localization system in the building, this system can be used for crowd-sourcing. In the crowd-sourcing system, the airflow values along with the location will be sent to a central server, that can be used by the building management system to understand the air circulation in the building. This way we can create an application where users can see which building has better air circulation and make an informed decision.

\textit{Limitations and Future Work} The major limitation of the proposed system is that it does not give any information about the quality of airflow. In future, the information form this system can be combined with the air quality information to give a complete picture to the users. \names also does not give any information about the direction of airflow. In the future work, we plan to explore multiple microphones of the smartphones to estimate the direction of airflow as well by using beam-forming to identify the location of the source. We can also find the direction of airflow by leveraging smartphone orientation sensors. 
Another major limitation of this system is that certain ambient noises that are consistent and similar to airflow may affect the system accuracy.


\textbf{PAPER ENDS HERE!!!}
\iffalse

\noindent

\textbf{Device Considerations}
\subsubsection{Device Distances and Orientations}

The traditional forms of sensing airflow rates require devices to be installed near the air supply vent. This requirement, however, is impractical to ask of everyday users. In a room 3 meters high (from the surface of the floor to the ceiling vent), we vary the distance between the user's smartphone and ceiling vent. In an ideal scenario, a user be standing up and holding the smartphone in their hand while sensing - 1.5 meters away from the vent. It is also common for a user to conveniently place the device on the tabletop to sense for airflow - 2.25 meters away from the vent. Additionally, it is common for  In less ideal situations, users may need to extend their arm to position the smartphone closer to the vent; this will put the device 1 meter and 0.5 meters away from the vent, respectively.

Also notable is the changing ways users hold their phones. To ensure device orientation does not impact our application performance, our experiment accounts for the following orientation condition - 0 degrees (microphone faces vent), 90 degrees(microphone is rotated 90 degrees from facing vent), and 180 degrees (microphone faces the floor).

\fi

\noindent \textbf{Environment Considerations}
\subsubsection{Air Supply Vents}
It is possible that users are located in areas with different types of ventilation. To account for these variations, we introduce several air supply vents located in different room sizes and orientations for our experiment. Note that the rooms assume an economic workspace consideration of 100 square feet per employee. The details are as follow: V1 and V2 are ceiling vents located at two extreme ends of a private room for one person, \missing{V3 is a wall vent in a mid-size room for six persons, V4 is a ceiling vent in a private room for one person, and V5 is a ceiling vent in a mid-size room for six persons. Except for V4, which is located in an older facility, all vents are within the same building.}

\begin{figure}
    \centering
    \includegraphics[width = 0.7\columnwidth]{Screen Shot 2021-08-30 at 14.26.04.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

\subsubsection*{Environment Considerations}

\begin{table} [ht!]
\begin{tabular}{|c|c|l|c|}\hline
\textbf{Vent} & \textbf{Type} & \textbf{Room-size} & \textbf{Acc.}\\ \hline
V1 & ceiling & 1 pax, private room & XXX \\
V2 & ceiling & 1 pax, private room as V1 & XXX \\
V3 & wall & 6 pax, mid-size room & XXX \\
V4 & ceiling & 1 pax, private room (old building) & XXX \\
V5 & ceiling & 6 pax, mid-size room & XXX \\ \hline
\end{tabular}%} 
\caption{Accuracy, measured in MSE, of \names on various smartphone distances and orientations. }
\label{tab:smartphone_venttype}
\end{table}


\iffalse
Regression model trained on Smartphone

20000 data points - 80-20 train-test split.
Results shown in Table 1

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
         & Regression Score & MSE \\
         \hline
       Train  & 0.9915 & 0.4738\\
       \hline
     Test &    0.9437 & 3.0836\\ \hline
    \end{tabular}
    \caption{Smartphone-trained regresssion model}
    \label{tab:my_label}
\end{table}

\begin{enumerate}
    \item Additional challenges: placement and orientation problems

    \begin{table}[]
        \centering
        \begin{tabular}{|c|c|}
         \hline \textbf{Distance(m)}   &  \textbf{Test MSE} \\ \hline
          0.5   & 1.3484 \\ \hline
          1 & 1.7282 \\ \hline
          1.5 & 5.8955 \\ \hline
          
        \end{tabular}
        \caption{Effect of distance on accuracy}
        \label{tab:my_label}
    \end{table}
    
    
    
    \begin{table}[]
        \centering
        \begin{tabular}{|c|c|}
         \hline \textbf{Orientation(degrees)}   &  \textbf{Test MSE} \\ \hline
          0   & 1.7707 \\ \hline
          90 & 2.2001 \\ \hline
          180 & 2.0984 \\ \hline
          
        \end{tabular}
        \caption{Effect of orientation on accuracy}
        \label{tab:my_label}
    \end{table}
    
    
    \item phone moving - accelerometer (moving - dont collect the phone)
    \item position is well suited -  to use the proximity sensor, will tell the context, is it exposed, facing upward. if in a way to collect data, then collect
    \item battery efficiency: first of all need to sample every few minutes, it turns on to find a k-sample. for 1 second every 5 minutes
\end{enumerate}
\fi

==> smartphone_old.tex <==
\section{Case Study: Smartphone Implementation}
\label{sec:casestudy}
In this section, we extend our efforts to realizing \names as a smartphone application (Android) solution. We demonstrate the ability of \names to perform for everyday users.

%\begin{figure}[ht!]
%    \centering
%    \includegraphics[width=120mm]{figures/mobilesystem.jpg}
%    \caption{\names mobile application.}
%    \label{fig:mobilesys}
%\end{figure}

\subsection{Implementation}
Most smartphone microphone recorders running on Android devices capture audio signals at a minimum sampling rate of 16 kHz. By taking every 16\textsuperscript{th} sample from the microphone buffer, we effectively create a 1 kHz sampling rate of the audio samples needed for our app. In doing so, we bear the advantage of minimizing computation to only low-frequency components and isolating the FFT results to be within the range of 0-500 Hz, which is more privacy preserving. 

\begin{figure}[ht!]
    \centering
    \includegraphics[width=80mm]{figures/phonesetup.jpg}
    \caption{\names mobile application running on devices, P1 for collecting ground truth and P3 for real-time airflow prediction.}
    \label{fig:mobilesetup}
\end{figure}

We utilized \emph{Noise}, a widely available FFT computation library on \emph{kissfft} implementation \todo{[XXX]}. The FFT uses 16 samples for each calculation. An FFT of size 16 of a signal sampled at 1 kHz will result in a frequency resolution of 62.50 Hz, as required by our trained model. Additionally, we leverage the \emph{JPMML-Evaluator} library to compute predictions from our trained model directly on the smartphone \todo{[XXX]}. Our implementation and dataset are available on [redacted].

\subsubsection*{Ground Truth Setup}
Refer to Figure \ref{fig:mobilesetup}. We utilized a smartphone device, P1 (LG Stylo 4, Snapdragon 450 @ 1.8 GHz, 2GB RAM) to build a trained model. P1 is simultaneously paired with an Arduino Nano 22 BLE sense and the Rev. P wind sensor (same as our device setup in the Feasibility study, Section \todo{XXX}) to collect the airflow readings for ground truth. 

\subsection{User Considerations}
The implementation of \names as a mobile application for everyday users comes with several device and environment considerations. In conducting our case study, our goal is to understand how \names performs under the following conditions:\\

\noindent \textbf{Device Considerations}
\subsubsection{Device Distances and Orientations}
-choosing 1 main vent and testing on diff orientation and distances

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{bar_plot_with_error_bars.png}
    \caption{Device distance and orientations}
    \label{fig:my_label}
\end{figure}


- vent status, extending the limit where acc of classifying vent status significantly drops. Currently, exp. is tested 2.5m max.
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
        Distance(m) & Train Accuracy & Test Accuracy & Precision & Recall  \\ \hline
        0.5 & 0.999 & 0.978 & 0.983 & 0.974  \\ \hline
        1 & 0.997 & 0.962 & 0.965 & 0.958  \\ \hline
        1.5 & 0.996 & 0.959 & 0.960 & 0.958  \\ \hline
        0.5 & 0.986 & 0.938 & 0.940 & 0.937  \\ \hline
        
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}



The traditional forms of sensing airflow rates require devices to be installed near the air supply vent. This requirement, however, is impractical to ask of everyday users. In a room 3 meters high (from the surface of the floor to the ceiling vent), we vary the distance between the user's smartphone and ceiling vent. In an ideal scenario, a user be standing up and holding the smartphone in their hand while sensing - 1.5 meters away from the vent. It is also common for a user to conveniently place the device on the tabletop to sense for airflow - 2.25 meters away from the vent. Additionally, it is common for  In less ideal situations, users may need to extend their arm to position the smartphone closer to the vent; this will put the device 1 meter and 0.5 meters away from the vent, respectively.

Also notable is the changing ways users hold their phones. To ensure device orientation does not impact our application performance, our experiment accounts for the following orientation condition - 0 degrees (microphone faces vent), 90 degrees(microphone is rotated 90 degrees from facing vent), and 180 degrees (microphone faces the floor).

\subsubsection{Device Model Variations}
Smartphone device models can cause variation in application performance. To ensure \names performs the same way for different user devices, our experiment comprises two additional smartphone devices for testing, P2 and P3. The specifications are as follow: P2 - LG Stylo 3, Snapdragon 435 @ 1.4 GHz, 2GB RAM. P3 - Google Pixel XL, Snapdragon 821 @ 2.15 GHz, 4GB RAM.\\

\noindent \textbf{Environment Considerations}
\subsubsection{Air Supply Vents}
It is possible that users are located in areas with different types of ventilation. To account for these variations, we  introduce several air supply vents located in different room sizes and orientations for our experiment. Note that the rooms assume an economic workspace consideration of 100 square feet per employee. The details are as follow: V1 and V2 are ceiling vents located at two extreme ends of a private room for one person, \todo{V3 is a wall vent in a mid-size room for six persons, V4 is a ceiling vent in a private room for one person, and V5 is a ceiling vent in a mid-size room for six persons. Except for V4, which is located in an older facility, all vents are within the same building.}

\begin{figure}
    \centering
    \includegraphics[width = 0.7\columnwidth]{Screen Shot 2021-08-30 at 14.26.04.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}


\subsubsection{Noise-Level in Room}
Recall Section \ref{sec:sampleperiod}. We listed the potential scenarios to which our system will be utilized and respond. We broadly categorize indoor situations users are likely to be in; (a) a mid-sized room with several humans conversing (e.g., a meeting), (b) a crowded large-sized room with a distinct speaker (e.g., conference), and (c) a crowded large-sized room with multiple ongoing conversations (e.g., cafeteria). As a final step, we evaluate \names under different noise levels, representing the three scenarios described.
\begin{figure}
    \centering
    \includegraphics[width = 0.5\columnwidth]{Screen Shot 2021-08-30 at 14.29.31.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}


\subsection{Results}
\subsubsection*{Device Considerations}
Table \ref{tab:smartphone_distorient} tabulates the accuracy of \names on different distances and orientations, as described above. In an ideal situation where a user stands up and holds the phone in their hand, \names achieve a low mean squared error between 1.54-1.77. The consistency of the accuracy, however, fluctuates more with distance. \ncz{how is phone placed on a table with its screen facing upwards giving higher MSE than microphone pressed down on the table?}

\begin{figure}[h!]
\begin{minipage}[h]{.45\linewidth}
\centering
%\scalebox{0.7}{
\begin{tabular}{|l|c|c|c|c|}\hline
\textbf{Dist/Orient.} & \textbf{0.5m} & \textbf{1.0m} & \textbf{1.5m} & \textbf{2.25m} \\ \hline
0 degrees  & 0.85 & 1.77 & 4.22 & 5.88 \\ 
90 degrees  & 1.75 & 1.59 & 1.77 & 4.67 \\ 
180 degrees & 0.93 & 1.49 & 1.54 & 1.81 \\ \hline
\end{tabular}%} 
\caption{Accuracy, measured in MSE, of \names on various smartphone distances and orientations. }
\label{tab:smartphone_distorient}
\end{minipage}\hfill
\begin{minipage}[h]{.5\linewidth}
\centering
%\scalebox{0.7}{
\begin{tabular}{|l|c|c|c|}\hline
 & \textbf{P1} & \textbf{P2} & \textbf{P3}  \\
  & LG Stylo 4 & LG Stylo 3 & Google Pixel XL  \\ \hline
\textbf{Acc.} & XXX & XXX & XXX \\ \hline
\textbf{Time} & 3.1 ms &  3.4 ms &  2.9 ms \\ \hline
\end{tabular}%}     
\caption{Accuracy (in MSE) and processing time (in milliseconds) of \names on three smartphone models. }
\label{tab:smartphone_model}
\end{minipage}
\end{figure}

In these experiment runs, all phones are assumed stationary. We recommend coupling the app with context-aware capabilities sensing for user activity, phone exposure, and device orientations in a full-fledged implementation. For example, essential movement detection or the phone being stationary can be known using an accelerometer, while phone exposure can be known using proximity and light sensors. \names will not sense unless the necessary conditions of the device being stationary, exposed, and adequately oriented are met.

Next, Table \ref{tab:smartphone_model} lists \ncz{results for smartphone variation?} 

\begin{enumerate}
    %\item Additional challenges: placement and orientation problems
    %\item phone moving - accelerometer (moving - dont collect the phone)
    %\item position is well suited -  to use the proximity sensor, will tell the context, is it exposed, facing upward. if in a way to collect data, then collect
    \item battery efficiency: first of all need to sample every few minutes, it turns on to find a k-sample. for 1 second every 5 minutes
    %\item screenshot of app
\end{enumerate}

\subsubsection*{Environment Considerations}

\begin{table} [ht!]
\begin{tabular}{|c|c|l|c|}\hline
\textbf{Vent} & \textbf{Type} & \textbf{Room-size} & \textbf{Acc.}\\ \hline
V1 & ceiling & 1 pax, private room & XXX \\
V2 & ceiling & 1 pax, private room as V1 & XXX \\
V3 & wall & 6 pax, mid-size room & XXX \\
V4 & ceiling & 1 pax, private room (old building) & XXX \\
V5 & ceiling & 6 pax, mid-size room & XXX \\ \hline
\end{tabular}%} 
\caption{Accuracy, measured in MSE, of \names on various smartphone distances and orientations. }
\label{tab:smartphone_venttype}
\end{table}

\begin{table} [ht!]
\begin{tabular}{|l|c|c|}\hline
\textbf{Environment} & \textbf{Speech/Noise-level} & \textbf{Acc.}\\ \hline
Three way conversation in a meeting room & Audible & XXX \\
Speaker to an audience in a seminar room & Audible & XXX \\
Busy restaurant & White noise & XXX \\ \hline 
\end{tabular}%} 
\caption{Accuracy, measured in MSE, of \names on various smartphone distances and orientations. }
\label{tab:smartphone_speechtype}
\end{table}
\ncz{stopped here!}

\begin{figure}
    \centering
    \includegraphics[width=5cm,height=10cm]{app.png}
    \caption{Android Application}
    \label{fig:my_label}
\end{figure}

Regression model trained on SmartPhone

20000 data points - 80-20 train-test split.
Results shown in Table 1

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
    \hline
         & Regression Score & MSE \\
         \hline
       Train  & 0.9915 & 0.4738\\
       \hline
     Test &    0.9437 & 3.0836\\ \hline
    \end{tabular}
    \caption{Smartphone-trained regresssion model}
    \label{tab:my_label}
\end{table}

\begin{enumerate}
    \item Additional challenges: placement and orientation problems

    \begin{table}[]
        \centering
        \begin{tabular}{|c|c|}
         \hline \textbf{Distance(m)}   &  \textbf{Test MSE} \\ \hline
          0.5   & 1.3484 \\ \hline
          1 & 1.7282 \\ \hline
          1.5 & 5.8955 \\ \hline
          
        \end{tabular}
        \caption{Effect of distance on accuracy}
        \label{tab:my_label}
    \end{table}
    
    
    
    \begin{table}[]
        \centering
        \begin{tabular}{|c|c|}
         \hline \textbf{Orientation(degrees)}   &  \textbf{Test MSE} \\ \hline
          0   & 1.7707 \\ \hline
          90 & 2.2001 \\ \hline
          180 & 2.0984 \\ \hline
          
        \end{tabular}
        \caption{Effect of orientation on accuracy}
        \label{tab:my_label}
    \end{table}
    
    
    \item phone moving - accelerometer (moving - dont collect the phone)
    \item position is well suited -  to use the proximity sensor, will tell the context, is it exposed, facing upward. if in a way to collect data, then collect
    \item battery efficiency: first of all need to sample every few minutes, it turns on to find a k-sample. for 1 second every 5 minutes
    \item screenshot of app
\end{enumerate}

==> system.tex <==
\section{\name: Our Proposed Solution}
\label{sec:system}
In this section, we introduce our proposed system, \name. Figure \ref{fig:sysOverview} illustrates the system overview, predicting two airflow characteristics, namely, the state of air vents and the rate of airflow. Note that our project consisting of datasets, models, and visualizations are available for researchers alike. These resources can be accessed through: [link redacted].

\begin{figure}[!h]
\centering
    \includegraphics[width=\linewidth]{final_figures_only/system.jpg}
    \caption{System overview of \name, consisting of three components.}
    \label{fig:sysOverview}
\end{figure}

\subsection{Pre-Processing Module}
We begin by capturing audio signals from the microphone signal at 16 kHz. We based this decision on our review of smartphone specifications, where the lowest standard native sampling frequency across modern Android and iOS phones is 16 kHz. The primary function of our pre-processing module ensuring user privacy and remove high frequencies and ambient noise from the signal. We achieve this goal in three steps: First, the module divides the audio signal into segments of $n$ ms \missing{<to ... explain why>}. Second, it employs a silent-period detection algorithm, which iteratively discards audio clips that contain audible human speech (see Section \ref{sec:silentperiods}). Thus, we only process the signal further if it is detected as silent period i.e. not having high ambient noises. 
%Note, however, that the clips it continues to process may still contain high amounts of ambient noises and possibly lower frequency human voices as left behind residue. 
Finally, it applies a low pass filter to remove high frequency noises. As we will discuss in Section \ref{sec:feasibility}, our experiments found the optimal cut-off frequency of the low pass filter at 375 Hz.


\subsection{Feature Extractor}
Our second module takes in non-human-audible low-frequency audio clips to compute features. Specifically, the feature extractor applies a Fast Fourier Transform(FFT) to the input data, converting the signal from the time domain to the frequency domain. Like many real-time digital signal processing applications, the FFT must be computed on a shorter duration. As discussed in Section \ref{sec:feasibility},  we set the FFT sample size to 256, resulting in a window size of 256/16000 = 0.016 seconds. 16 ms of signal data is short enough duration to produce a total of seven frequencies and their corresponding amplitudes as features for our models.

\missing{For the label, we use an airflow sensor rev.p by modern devices. The airflow value received from the airflow sensor is used as the label and logged in the file along with the features. }

\subsection{Prediction Module}
We employ standard machine learning techniques to predict mainly two characteristics of airflow: (1) The state of an air vent, as a binary classification problem predicting a discrete class label of the vent on or off and (2) The rate of airflow, as a regression problem to predict the continuous values of airflow coming from the air vent.

\begin{wrapfigure}{r}{.5\linewidth}
\centering
\scalebox{.75}{
\begin{minipage}{\linewidth}
\begin{algorithm}[H]
\caption{Minimum Persistent Scheme(MPS) }\label{alg:euclid}
\begin{algorithmic}[1]
\State Initialize $n$, $\epsilon$, $p$

\Procedure{MinimumPersistingValue}{$arr$}\Comment{$arr$ is list of n consecutive predictions}
\State $arr \gets sort(arr)$
\State $per \gets [arr[0]]$ \Comment{initialize the persistence window with the 1st element}
\State $i\gets 1$
\While{$i\not=n$}
\If{$abs(mean(per)-arr[i]) <= \epsilon$}
    \State $per.append(arr[i])$
% \Else
%     \State $y \gets y \times X$
%     \State $N \gets N - 1$
\ElsIf{$abs(mean(per)-arr[i]) > \epsilon$}
    \State $per \gets [arr[i]]$ \Comment{if this element deviates by more than $\epsilon$, start a new window}
% \Else
%     \State $y \gets y \times X$
%     \State $N \gets N - 1$
\EndIf
\If{$length(per) = p$}
    \State return $mean(per)$
\EndIf

\State $i\gets i+1$
\EndWhile
\State return \textbf{failure}
\State
\EndProcedure

% \State $\mu, \sigma = gp.predict(grid)$\Comment{$\mu$ and $\sigma$ are matrices}
% \State \textbf{return} $argmax(\mu + \sigma * \sqrt\beta)$\Comment{UCB aquisition function}

\State $i\gets 0$, $arr[n]$
\While{$i\not=n$}
\State Get $p\_value$\Comment{$p\_value$ is the predicted value given by the model}
\State $arr.append(p\_value)$
\State $i\gets i+1$
\EndWhile

\State MPV = MinimumPersistingValue(arr)
\end{algorithmic}
\end{algorithm}
\end{minipage}%
}
\end{wrapfigure}

Prior studies set in the context of sensing breathing patterns have been proposed to utilize \missing{<classifier 1> and <classifier 2> [cite several works]}.  These findings inform our decision to similarly investigate the effectiveness of these classifiers in the context of predicting airflow. Our results in Section \missing{XXX} demonstrate the applicability of these models to predict airflow. We show how the Gradient Boosting model outperforms other techniques in solving both our classification and regression problems. 

A significant part of our regression model is driven by our proposed technique of the Minimum Persistent Scheme (MPS, see Section \missing{XXX}). This function mainly helps improve our model accuracy by removing the effects of ambient noises in the low-frequency range, which may inadvertently be processed—refer to Algorithm \missing{XXX} for the pseudo algorithm of MPS.


%- subsec2:description of data you're processing

%The classification model predicts the state of the vent so it has label 1(on) or 0(off). 

%-subsec3. - why these models graph and why xgboost



%Keep referencing the figure

\iffalse
\subsubsection*{Model Architecture for Classification}
%\todo{redo - separate result from description}

We use an XGBoost classifier with the following parameters:
n\_estimators: 500,
          max\_depth: 5,
          min\_samples\_split: 5,
          learning\_rate: 0.2




\subsubsection*{Model Architecture for Regression}
\missing{redo - separate result from description}
For the regression model, we use an airflow sensor to label each data point with airflow in meters per second. We recorded data from different distances and different orientations of microphone. We run a XGBoost regression model on this data. XGBoost is an optimized distributed gradient boosting library designed to be highly efficient, flexible and portable. It implements machine learning algorithms under the Gradient Boosting framework. XGBoost provides a parallel tree boosting (also known as GBDT, GBM) that solve many data science problems in a fast and accurate way. 

\fi

==> technique.tex <==
\section{Technique}
Indeed, narrowing our data source to only audio signals would require our solution to rely on a combination of several techniques. 



\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.4\columnwidth]{figures/humanTypeNoise_placeholder.jpg}
    \caption{Diagram shows how low frequency audio signal of moving air in a room differentiates itself from typical human noises.}
    %\vspace{-4mm}
    \label{fig:technique_humannoise}
\end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.5\columnwidth]{figures/airflow_spectrum.png}
    \caption{Frequency spectrum of microphone signal with vent on in the room at a distance of 2.25 m (at desk)}
    %\vspace{-4mm}
    \label{fig:spectrum_air}
\end{figure}




\subsection{Eliminating the effect of Ambient Noise}

After passing the microphone signal through a low pass filter of 375 Hz, we observe that privacy is no longer a concern for the system performance as shown in the user study in section 6.2.4. But ambient noise is affecting the system accuracy because there is an overlap between airflow signal and the audible frequencies, thus airflow and audible frequency spectrum are not mutually exclusive. Thus, the audible frequencies between 20-375 Hz will affect the system performance. Out of which, human speech has a a fundamental frequency of 300Hz and a maximum frequency of 8kHz\cite{titze1998principles}a fundamental frequency from 300Hz and a maximum frequency of 8kHz. Thus, ambient noise will interfere with the airflow signal and degrade the system performance as observed in Figure \ref{fig:RMS}. One key observation in this Figure is that airflow is continuous signal with approximately constant amplitude and does not change much with time. Whereas other ambient noises like talking, coughing, and background noises are discrete and change a lot with time. We use this key observation and propose two techniques to solve this challenge:
%When the ambient noise is high(represented by RMS value), the predicted airflow is high. This is because the model learned that the amplitude of the low frequency band is high when rate of airflow is high. This means that ambient noise leads to incorrect airflow predictions. To address this challenge, we use two techniques. 

%Add a figure

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/RMS_prediction.png}
    \caption{RMS power value of microphone signal with predicted and actual airflow }
    %\vspace{-4mm}
    \label{fig:RMS}
\end{figure}

%Add a spectrum of airflow with ambient noise with proper labelling of frequency

\subsubsection{Sampling in Silent periods}
To address the challenge of ambient noise affecting the system accuracy, we use silent period detection based sampling technique because this problem is due to the interference of audible noise in the spectrum-of-interest. The intuition is that we will run our model only when there is minimum ambient noise in the environment and discard the sample otherwise. In this approach, we find the root mean squared(RMS) value of the power of microphone signal and compare it with a threshold to detect silent periods. If a silent period is detected, we run our model and predict airflow and state of the vent. Otherwise, we discard the sample. Then, we only sample during these silent periods. This increases system accuracy significantly as we are not sampling during high levels of ambient noise which leads to incorrect predictions and misclassifications. Another important aspect that we study is the percentage of silent periods which is the ratio of number of silent periods to the sum of silent periods and non-silent periods for a given duration of time. Sampling in silent periods means that we are not reporting airflow as frequency as we were before. This frequency will further reduce in presence of loud crowd noise. To quantify this, we present a study to show that based on our threshold and window size, there are sufficient percentage of silent periods that can be used to predict airflow or state of vent. Also, since the airflow does not change very frequently, we do not need the airflow reading very often. Silent-period Sampling offers an added advantage of further ensuring privacy of the system.\\
%We have implemented the system on the smartphone that labels each data point as 0(non-silent period) or 1(silent period). 
\textit{Threshold Selection}: The major problem in realizing this technique is threshold selection. 
%A threshold should be selected such that it is the maximum decibels of noise that can come from a vent anything above that can be discarded.  
We identify some potential thresholds by empirically observing the maximum RMS value that can be generated from the vent. Then, we perform a experiment and we observe the percentage accuracy improvement(with and without silent period based sampling) and percentage of silent periods for each threshold. We choose the threshold that performs best on both metrics. 



%To continuously sample for airflow will only introduce unnecessary computation costs and more significant privacy concerns. From a technical standpoint, we must first determine the appropriate time to sample for audio signals. When a chance to sample exists, we must then decide the optimal sampling component and sampling rate to predict.

The potential scenarios to which our system will be utilized and respond are only for indoor environments. However, the noise levels can drastically change with occupancy during the course of the day. Figure \ref{fig:noisegap_spectrum} illustrates the audio signals of three broadly categorized indoor situations involving human speech we expect to encounter: (a) a mid-sized room with several humans conversing (e.g., a meeting), (b) a crowded large-sized room with a principal speaker (e.g., conference), and (c) a crowded large-sized room with multiple ongoing conversations (e.g., cafeteria).



From Scenarios \ref{fig:noisegap_spectrum}(a) and (b), we observe structures of pauses that commonly exist in conversations. However, these ``silent gaps'' are less apparent in processing audio signals for Scenario (c).  

%A preliminary analysis of these audio signals found distinct gaps from as much as ten seconds to as little as ten milliseconds (ms). Figure \ref{fig:technique_label} illustrates the number of 16 ms gaps in Scenario (a), specifically 158 silent periods. These periods cumulatively result in approximately 15\% of a 26-second audio clip, and the lowest possible sample will be -96 dBFS. Assuming 0 dBFS is the highest audio level, we believe that setting the silent threshold closer to -96 dBFS will increase our chances of sampling without human audible information. 
In Section 6.2.4, we conduct experiments in our feasibility study to determine an optimal threshold for these silent gaps to accurately predict airflow and the percentage of silent periods in usual conversations. 
%However brief they may be, our technique must first work by anticipating notable pauses as a desired data collection period to preserve user privacy.

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/silence.png}
    \caption{Replace diagram that zooms into 1-3 silence periods so as to see clear difference in audio signals.}
    \label{fig:technique_silencegap}
\end{figure}



% Threshold selection


\subsubsection{Minimum Persistent Scheme}

%Why is Silent-period detection not sufficient?
Although the silent period based technique improves the system accuracy significantly in presence of ambient noise, it still suffers from the problem of being a threshold-based technique. It may happen that the sensor detects some non-silent periods as silent periods because the threshold is set to be the upper bound of silence. So, if ambient noise decibel levels are very low(comparable to airflow noise), the system will consider it as a silent period as the system is simple using decibel-based thresholding. So, we propose another technique that further improves system accuracy against ambient noises and makes it more robust. This algorithm runs only on the regression model after the prediction has been made.

While evaluating the \names regression model in the presence of ambient noise, we observe that common types of ambient noise such as voices, music, or other environmental sounds cause the regression model to exclusively \emph{overpredict} rates of airflow in the environment. This is because the model has learned that the amplitude of low frequency spectrum indicates that magnitude of airflow.
%The presence of airflow has no effect on the percentage of regression predictions which are below the ground truth value. 
From a noise perspective, we also notice that airflow is a continuous signal and ambient noise is discrete -- it happens in bursts. We can use these combined properties to estimate airflow correctly even in the presence of ambient noise. All we need to do is find the minimum persisting airflow prediction out of n consecutive predictions. We are finding minimum value based on our observation that ambient noise leads to over-prediction and persisting value because airflow is continuous and its magnitude does not change very much with time.

First, we notice that when ambient noise is present, there are millisecond-scale "silent periods" in the audio signal.  Because \names samples represent short durations of time, we can reasonably expect that during a stream of continuous samples, many of the samples will have been entirely sampled during one of these silent periods.  With the knowledge that ambient noise causes the regression model to overpredict, we consider an algorithm that takes as input some sequence of continuous samples, of size $n$.  Since we are only interested in the points where ambient noise is not present, we conjecture that reporting the minimum prediction obtained from the $n$ samples would be an accurate representation of airflow. 

In practice, however, simply reporting the minimum predicted value greatly increases the effect of \emph{outlier values}, which may in fact under predict the ground truth airflow value.  Thus, we introduce two parameters persistance parameter $p$ and threshold parameter $\epsilon$ which capture some measure of \emph{persistence} in the predictions.  Considering the same sequence of $n$ numbers, we propose an algorithm which sorts the predictions in ascending order, and subsequently attempts to find a "window" of values with size $p$, such that $p$ consecutive values are all within $\pm \epsilon$ of the window's average value.  The algorithm then reports this average value as the prediction for all $n$ samples, or, if such a window cannot be found, simply terminates and waits to receive a new batch of $n$ samples.  In Fig. \ref{fig:MinPer}, we show that these minimum persistent post-processing of predictions yields much better accuracy compared with a naive approach that omits any processing. Thus, MPS is an additional features that characterizes the properties of airflow signal to make better predictions, thus increasing system accuracy.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.6\columnwidth]{minper.png}
    \caption{Minimum Persistent accuracy improvement on real test data with background ambient noise, 2 person conversation.}
    \label{fig:MinPer}
\end{figure}

\iffalse
\subsection{Sampling Period}
\label{sec:sampleperiod}
To continuously sample for airflow will only introduce unnecessary computation costs and more significant privacy concerns. From a technical standpoint, we must first determine the appropriate time to sample for audio signals. When a chance to sample exists, we must then decide the optimal sampling component and sampling rate to predict.

The potential scenarios to which our system will be utilized and respond are only for indoor environments. However, the noise levels can drastically change with occupancy during the course of the day. 



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/silence.png}
    \caption{Replace diagram that zooms into 1-3 silence periods so as to see clear difference in audio signals.}
    \label{fig:technique_silencegap}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{DC (1).png}
    \caption{Another possible way is to duty Cycling the low pass filtered signal}
    \label{fig:DC}
\end{figure}

\subsection{Filtering and Sampling}
\ncz{sensing 16ms for n seconds - explain how to get n seconds}
\ncz{deciding on -45dBFS was based on app? need more analysis on the optimal threshold for gap}
As presented in Section \ref{sec:air_low}, it is conceivable that the low-frequency component of moving air can be quickly separated from other noises through a low pass filter. The benefits of leveraging a low pass filter are two-fold. First, the low-pass filtering technique can eliminate less relevant samples to airflow and reduce unnecessary computation. Second, eliminating high-frequency components will discard much of the human speech, simultaneously reducing privacy risks, which would otherwise be processed for airflow prediction. In situations where complete silent periods are unavailable, filtering can be of benefit. 

Figure \ref{fig:soundconcept} illustrates the low frequency component of the microphone audio signal under several indoor conditions. By applying a Fourier-based algorithm to enhance the contrast of the signals, we can distinguish the spike in the frequency domain; the amplitude (a measurement of how large the wave is) becomes prominent when airflow pressure increases from the air supply vent. 

The natural course of action would be to assess the maximum audible low-pass cutoff frequency. Much work in speech-in-noise research has found speech energy beyond 8 kHz to remain audible for regular listeners \cite{monson2019maximum}. Hence, our technique must consider an optimal cutoff frequency leaving most speech results in a detectable loss and minimal possibility to reconstruct while ensuring sufficient samples of the low-frequency component for accurate prediction.

Low-frequency components remain vulnerable to the possibilities of data reconstruction and risking user privacy. To circumvent this risk, we can additionally sub-sample the data. By filtering and then subsampling, we avoid the situation where high-frequency components get aliased in the low-frequency band (Nyquist sampling theorem). \ncz{what do you mean by this: Also, we don't sample continuously and add delays to further enhance the privacy of the system. -- need more explanation to differentiate between sampling silent periods, subsampling and not sampling continuously.}


\fi

%\begin{figure}[ht!]
%    \centering
%    \includegraphics[width=\columnwidth]{FFT.png}
%    \caption{Fourier transform of microphone signal. \ncz{can we do this for noisy indoor setting?}}
    %\vspace{-4mm}
%    \label{fig:soundconcept}
%\end{figure}


